PAC-Learning Uniform Ergodic Communicative Networks

This work addressed the problem of learning a network with communication between vertices. The communication between vertices is presented in the form of perturbation on the measure. We studied the scenario where samples are drawn from a uniform ergodic Random Graph Process (RGPs for short), which provides a natural mathematical context for the problem of interest. For the binary classification problem, the result we obtained gives uniform learn-ability as the worst-case theoretical limits. We introduced the structural Rademacher complexity, which naturally fused into the VC theory to upperbound the first moment. With the martingale method and Marton's coupling, we establish the tail bound for uniform convergence and give consistency guarantee for empirical risk minimizer. The technique used in this work to obtain high probability bounds is of independent interest to other mixing processes with and without network structure.

==> sections/exactdeter.tex <==
% \subsubsection{Impossibility}
% From the definition we know that the Bayes estimator $T_B^*$ is admissible in $\fk T$ on the Bayes risk given prior $\fk P$. This being said, the impossibility conditions of exact Bayesian pair-wise ranking is the condition under which no strongly consistent Bayes estimator with respect to prior $\fk P\in\ca P$ exists. We formalize this observation through the following claim that can be directly obtained from definition.
% \begin{claim}[Sufficient Conditions]
% For some prior $\fk P$, if the Bayes estimator cannot exactly rank then no other estimators exactly rank.
% \end{claim}
% To apply our analysis, we first define automorphism on the group of vertices in weighted directed graphs.

% % \begin{definition}[Automorphism in Weighted Directed Graphs]
% % We say an automorphism $\pi\in\bb P$ on a weighted directed graph $G(\ca V,\ca E)$ with $\ca V=[n]$ is a permutation on $\ca V$ such that the graph $ G^\prime$ permuted according to $\pi$ from $G$ is isomorphic to $G^\prime(\ca V^\prime,\ca E^\prime)$ with $\ca E=\ca E^\prime$. The automorphisms in specific graph $G$ formed an automorphism group, which we termed \texttt{Auto}(G). In particular, the non-identity permutation in \texttt{Auto}(G) is termed non-trivial automorphism.
% % \end{definition}
% However, in the deterministic comparison setting, the notion of indistinguishable pair acts in more importance in our analysis. Intuitively, the automorphism is too strong a requirement for the WDGs to fulfill.
% \begin{definition}[Indistinguishable Pair]\label{lm:4}
% We say the indistinguishable pair $(i,j)$ with $i,j\in[n]$ and $i\neq j$ is an unordered pair of indices in a graph $G(\ca V,\ca E)$ such that for the graph $G^\prime(\ca V^\prime,\ca E^\prime)$ where $\ca V=\ca V^\prime$ and $\ca E^\prime=\ca E\setminus\{(i,j),(j,i)\}$, there exists $\pi\in$\texttt{Auto}($G^\prime$) such that $\pi(i)=j\wedge\pi(j)=i$.
% \end{definition}
% The following lemma is the basis of our result, which we give in increasing generality.
% % \begin{fact}\label{fac1}
% % Let $\ca A^m=\sum_{i=1}^m\bfa A_{i}$, then if the weighted directed graph induced by $\ca A^m$ has a non-trivial automorphism $\pi$ with $\pi(i)=j$, $\pi(j)=i$ and $\pi(k)=k$ for all $k\in[n]\setminus\{i,j\}$ with $\Theta(1)$ probability, the Bayes estimator will fail the requirement of exact recovery.
% % \end{fact}
% % \begin{lemma}\label{lm22}
% % If there exists a indistinguishable pair with $\Theta(1)$ in $G(\ca V,\ca E)$, then the exact pairwise ranking will be impossible.
% % \end{lemma}
% % \begin{proof}
% % We denote the following events \begin{compactenum}
% % \item $A_1:\ca A_{i,j}^m\geq \ca A_{j,i}^m$
% % \item $A_2: \ca A_{i,j}^m< \ca A_{j,i}^m$
% % \item $A_3: \exists\pi\in\text{Auto}(G^\prime)\text{ s.t. }\pi(i)=\pi(j)$
% % \end{compactenum}
% % By the conditions given in the lemma, we directly see that
% % \begin{equation*}
% %     \bfa P(A_1|A_3)=\Theta(1)\;\;\;\bfa P(A_2|A_3)=\Theta(1)
% % \end{equation*}
% % Hence with probability at least $\min\{\bfa P(A_1,A_3),\bfa P(A_2,A_3)\}$, any estimator will make mistake, making the exact ranking impossible.
% % \end{proof}
% \textbf{Discussion:} Although the exact ranking is impossible, the almost exact ranking was not affected here, which will require a stronger condition to make 
% With more involved analysis, the above fact can be further extended with the help of the notion of disagreement between vertices. 
% \begin{definition}[Disgreement between vertices]
% Let $\ca A$ be the adjacency matrix of a WDG denoted by $G(\ca V,\ca E)$. Let $i,j,k\in\ca V$ with $i\neq j$. Then we say $i,j$ disagree on $k$ in $G$ if $\ca A_{i,k}\neq \ca A_{j,k}$ or $\ca A_{k,i}\neq\ca A_{k,j}$
% \end{definition}
% % \begin{lemma}
% % With the same notations in Fact 1, 
% %  let $G(\ca V,\ca E)$ be the graph induced by $\ca A^m$ with $\ca V=[n]$. If the a pair $(i,j)$ with $i\neq j$ and  $i,j$ disagree on at most $O\bigg( \frac{m\log\frac{1}{\gamma_{min}}}{{\log \frac{n}{\sqrt{m}} +m\log 4}}\bigg)$ vertices in $G$ with probability $\Theta(1)$, the Bayes estimator will fail the exact ranking. 
% % \end{lemma}
% % \begin{proof}
% % The idea is to show that when there exists a pair $(i,j)$ that disagrees on $\ca A^m$ by less than $s$ vertices with probability $\Theta(1)$, the probability of mistaking $i$ with $j$ by Bayes estimator in the graph will be $\Theta(1)$.

% % Let $\ca V(G)$ be the vertex set of $G$. Let $\{k:i,j \text{ disagree on } k\text{ and } k\in[n]\setminus\{i,j\}\}=\ca S$. Let $G^\prime$ be the subgraph with $\ca V(G^\prime)=\ca V(G)\setminus\ca S$.

% % Consider the event $E_1(\ca S)$: there exists an non-trivial automorphism $\pi:[n]\setminus \ca S\rightarrow[n]\setminus \ca S$ in graph $G^\prime$ with  $\pi(i)=j,\pi(j)=i$ and $card(\ca S)= s$.


% % We denote the event that an automorphism exists in the graph $G$ by $E_2$. We can then introduce the state space of $E_2|E_1(\ca S)$ by $\bb X(E_2|E_1(\ca S))\subset\{0,1\}^{2\times s\times m}$. For any elements $\bfa X_{k,r,t}\in\bb X(E_2|E_1)$ we have $\left\{\begin{matrix}
% % \ca S_j\text{ wins over }\ca S_r \text{ at round } t  & \text{ if } \bfa X_{1,r,t}=1 \\
% % \ca S_i\text{ wins over }\ca S_r \text{ at round } t  & \text{ if } \bfa X_{0,r,t}=1 \\
% % \end{matrix}\right.$ 
% % Then the following estimate can be obtained:
% % \begin{align*}
% %     \bfa P(E_2|E_1(\ca S))&\geq \sum_{\bfa X \in\bb X(E_2|E_1(\ca S))}\prod_{t\in[m]} F_{\pi^*(i),\pi^*(r)}^{\bfa X_{0,r,t}}(1-F_{\pstr i,\pstr r}^{1-\bfa X_{0,r,t}})F_{\pstr j,\pstr r}^{\bfa X_{1,r,t}}(1-F_{\pstr j,\pstr r})^{\bfa X_{1,r,t}}\\
% %     &=\Omega(card(\bb X(E_2|E_1(\ca S)))\gamma_{min}^{2m}))
% % \end{align*}
% % Then we obtain the cardinality of $\bb X(E_2|E_1)$ by a simple combinatorial asymptotically as :
% % \begin{equation*}
% %     card(\bb X(E_2|E_1(\ca S)))=\bigg(\sum_{i=1}^m\binom{m}{i}^2\bigg)^s=\bigg(\binom{2m}{m}\bigg)^s=\Theta\bigg(\frac{4^{ms}}{\sqrt{m}^s}\bigg)
% % \end{equation*}
% % Hence we have:
% % \begin{equation*}
% %     \bfa P(E_2|E_1(\ca S))=\Omega(\gamma_{min}^{2m}\cdot \frac{4^{ms}}{\sqrt{m}^s})
% % \end{equation*}
% % Hence, using marginalization, we have:
% % \begin{align*}
% %     \bfa P(E_2)&=\sum_{\ca S}\bfa P(E_2|E_1(\ca S))\bfa P(\ca S)\\&=\Omega\bigg(\binom{n-2}{s}\cdot\gamma_{min}^{2m}\cdot \frac{4^{ms}}{\sqrt{m}^s}\bigg)\\
% %     &=\Omega\bigg(\bigg(\frac{(n-2)e}{s}\bigg)^s\cdot\gamma_{min}^{2m}\cdot \frac{4^{ms}}{\sqrt{m}^s}\bigg)
% % \end{align*}
% % By letting the R.H.S, be $\Theta(1)$, we prove the statement in the lemma.
% % \end{proof}
% %     \Pi_{MAP}(\bfa A_1^m)&=\argmax_{\pi\in\bb P}
% %     \bfa P(\pa A(\pi,\Pi^*)=1|\bfa A_1^m)\\
% %     &\propto\argmax_{\pi\in\bb P}\bfa P(\bfa A_1^m|\pa A(\pi,\Pi^*)=1)\bfa P(\Pi^*=\pi)
% % \end{align*}
% % \begin{align*}
% %     \Pi_{MAP}&=\argmin_{\eta:\bb A\rightarrow\bb P}\bb E[\bfa 1_{\Pi^*\neq\eta(\bfa A_1^m)}]
% % \end{align*}
% % We are interested in the Bayes risk, stated as follows:

% % \begin{align*}
% %     \bfa P(\pa A(\Pi_{MAP}(\bfa A_1^m),\Pi^*)=1)
% % \end{align*}
% % A general principal for MAP estimator ensured its optimality under the exact ranking requirement, which is implied by its definition. In other words, MAP stays at the fundamental limits of exact ranking requirement, formalized through the following theorem:
% With the above lemmas we can give the following theorem, which found a inner point on the impossibility region.

% % \begin{theorem}
% % A Bayes estimator failed exact ranking if:
% %     \begin{align*}
% %   m=\Omega\bigg(\max\bigg\{\bigg(\frac{\gamma_{max}}{\gamma_{min}}\bigg)^{4n},\frac{\log n}{n(\log 2+3\log\frac{\gamma_{min}}{\gamma_{max}}+\log\gamma_{min})}\bigg\}\bigg)
% % \end{align*}
% % % and
% % % \begin{equation*}
% % %     \log\frac{1}{\gamma_{min}}=o\bigg (\frac{\log n}{mn}+\log 2-\frac{\log m}{4m}\bigg )
% % % \end{equation*}
% % % with $\gamma_{min}=\inf_{w_i,w_j}F(w_i-w_j)$ and $\gamma_{max}=\sup_{w_i,w_j}F(w_i-w_j)$ which also suggests that any other estimator will fail exact ranking. 

% % % Moreover, when
% % % \begin{equation*}
% % %     \log\frac{1}{\gamma_{max}}=\Omega\bigg (\frac{\log n}{mn}+\log 2-\frac{\log m}{4m}\bigg )
% % % \end{equation*}
% % % then there exists no distinguishable pair in the induced WDG a.s.
% % \end{theorem}

% % \begin{proof}
% % We denote the ensemble of $\bfa A^m_1$ by $\ca{ A}^m$, namely
% %  \begin{equation*}
% %      \ca {\bfa A}^m_{i,j}=\sum_{k=1}^m\bfa A_{i,j}^k
% %  \end{equation*}
% % %  We further let $a_{i,j}^m=\sum_{k=1}^m A^m_{i,j}$.
% % By the definition of prior measure and the independence between upper right entries given $\Pi=\pi^*$, we have
% % \begin{align*}
% %     \bfa P(\bfa A_1^m)&=\prod_{i,j\in [n]\wedge j>i}\bfa P(\ca A_{i,j}^m)\\
% %     &=\prod_{i,j\in [n]\wedge j>i}\binom{m}{\ca A_{i,j}^m}F_{\pstr i,\pstr i}^{\ca A_{i,j}^m}(1-F_{\pstr i,\pstr i})^{m-\ca A_{i,j}^m}
% % \end{align*}
% % According to the Lemma \ref{lm22}, as long as we find a sufficient condition under which automorphism exists with probability $\Theta(1)$, the Bayes estimator will fail in exact ranking. Let $G(i,j)$ be the graph induced by $\ca A_{i,j}^m$. Denote the event $E_{i,j}$ as the existence of non-trivial automorphism $\pi$ on $G(i,j)$ such that $\pi( i)=j$ and $\pi(j)=i$. 

% % We define the state space of $E_{i,j}$ as $\bb X(E_{i,j})\subset\{0,1\}^{n\times n\times (m+1)}$. $\forall\bfa X\in\bb X(E_{i,j})$, we denote:
% % $\bfa X_{k_1,k_2,k_3}=1$ if party $k_1$ wins over $k_2$ in the $k_3$-th comparison. The following statement holds:
% % \begin{align*}
% %     \bfa P(E_{i,j})&=\sum_{\bfa X\in\bb X(E_{i,j})}\prod_{k\in[n]\setminus\{i,j\}}\bfa P(\ca A_{i,k}^m=\ca A_{j,k}^m)\\
% %     &=\sum_{\bfa X\in\bb X(E_{i,j})}\prod_{k\in[n]\setminus\{i,j\}}\prod_{c\in[m]} F^{\bfa X_{i,k,c}}_{\pstr i,\pstr k}\cdot(1-F_{\pstr i,\pstr k})^{1-\bfa X_{i,k,c}}\\
% %     &F_{\pstr j,\pstr k}^{\bfa X_{j,k,c}}(1-F_{\pstr j,\pstr k})^{1-\bfa X_{i,k,c}}
% % \end{align*}
% % summing over $i,j$, we have
% % \begin{align*}
% %     \mu_n&=\sum_{\{i< j\}\wedge\{ i,j\in[n]\}}\sum_{\bfa X\in\bb X(E_{i,j})}\prod_{k\in[n]\setminus\{i,j\}}\prod_{c\in[m]} F^{\bfa X_{i,k,c}}_{\pstr i,\pstr k}\cdot(1-F_{\pstr i,\pstr k})^{1-\bfa X_{i,k,c}}\\
% %     &F_{\pstr j,\pstr k}^{\bfa X_{j,k,c}}(1-F_{\pstr j,\pstr k})^{1-\bfa X_{i,k,c}}
% % \end{align*}
% % Here we introduced the notation $\inf_{i\leq j}F_{i,j}=\gamma_{min}$, with $1-\gamma_{min}=\gamma_{max}$ being the minimum probability and maximum probability respectively. We then estimate the asymptotic rate of $\mu_n$. Ignoring constant factors, the number of summands is roughly
% % \begin{equation*}
% %     \Omega( n^2\cdot card(\bb X(E_{i,j}))\gamma_{min}^{2mn})
% % \end{equation*}
% % where 
% % \begin{align*}
% %     card(\bb X(E_{i,j}))&=\bigg(\sum_{i=0}^m\binom{m}{i}^2\bigg)^{n-2}=\bigg(\sum_{i=0}^m\binom{m}{i}\binom{m}{m-i}\bigg)^{n-2}\\
% %     &=\binom{2m}{m}^{n-2}=\Theta\bigg(\bigg(\frac{4^m}{\sqrt{m}}\bigg)^{n-2}\bigg)
% % \end{align*}
% % where we used the fact that the coefficient of $m$-th order term of the following polynomial 
% % $
% %     (1+x)^m(1+x)^m
% % $
% % is exactly the sum enclosed by the big bracket. This leads to 
% % \begin{equation*}
% %     \mu_n^2=\Omega\bigg(n^4\cdot\bigg(\frac{4^m}{\sqrt{m}}\bigg)^{2n-4}\gamma_{min}^{4mn}\bigg)
% % \end{equation*}

% % Then we discuss over the joint event of $E_{i,j}\cap E_{k,l}$. There are two types of joint events that are correlated. 
% % \begin{compactenum}
% % \item $card(\{i,j,k,l\})=3$. Without loss of generality, we denote the two pairs by $(i,j)$ and $(j,k)$. The event implies that for all $l\in[n]\setminus\{i,j,k\}$, $\ca A^m_{i,l}=\ca A^m_{j,l}=\ca A^m_{k,l}$ and $\ca A_{i,j}^m=\ca A_{k,j}^m$.
% % \item $card(\{i,j,k,l\})=4$. This condition implies that for all $o\in[n]\setminus\{i,j,k,l\}$, $\ca A^m_{i,o}=\ca A^m_{j,o}=\ca A^m_{k,o}=\ca A^m_{l,o}$ and $\ca A^m_{i,l}=\ca A^m_{i,k}=\ca A^m_{j,k}=\ca A^m_{j,l}$
% % \end{compactenum}
% % In the first regime, we can write the probability of joint events of regime 1 as:
% % \begin{align*}
% %     \bfa P(E_{i,j}\cap E_{j,k})&=\bfa P(\ca A^m_{k,j}=\ca A_{i,j}^m)\prod_{l\in[n]\setminus\{i,j,k\}}\bfa P(\ca A^m_{i,l}=\ca A^m_{j,l}=\ca A^m_{k,l})\\
% %     &=\big(\sum_{\bfa X\in\bb X(\ca A^m_{k,j}=\ca A_{i,j}^m)}\prod_{c\in[m]}F_{i,j}^{\bfa X_{i,j,c}}(1-F_{i,j})^{1-\bfa X_{i,j,c}}F_{k,j}^{\bfa X_{k,j,c}}(1-F_{k,j})^{1-\bfa X_{k,j,c}}\big)\\
% %     &\cdot\big(\prod_{l\in[n]\setminus\{i,j,k\}}\sum_{\bfa X\in\bb X(\ca A^m_{i,l}=\ca A^m_{j,l}=\ca A^m_{k,l})}\prod_{c\in[m]}F_{j,l}^{\bfa X_{j,l,c}}(1-F_{j,l})^{1-\bfa X_{j,l,c}}\\&
% %     F_{i,l}^{\bfa X_{i,l,c}}(1-F_{i,l})^{1-\bfa X_{i,l,c}}F_{k,l}^{\bfa X_{k,l,c}}(1-F_{k,l})^{1-\bfa X_{k,l,c}}\big)\\
% %     &=\Theta\bigg(\binom{2m}{m}\bigg(\sum_{i=0}^m\binom{m}{i}^3\bigg)^{n-3}\gamma_{max}^{2m+3m(n-3)}\bigg)\end{align*}
% %     Using the inequality that for $x_i\geq 1$ for all $i\in[n]$:
% %     \begin{equation*}
% %         (\sum_{i}^n x_i^2)^3\geq(\sum_{i}^nx_i^3)^2
% %     \end{equation*}
% %     we obtain that
% %     \begin{equation*}
% %         \sum_{i=0}^m\binom{m}{i}^3\leq\binom{2m}{m}^{3/2}
% %     \end{equation*}
% %     Hence
% %     \begin{equation*}
% %         \bfa P(E_{i,j}\cap E_{j,k})=O\bigg(\bigg(\frac{4^m}{\sqrt m}\bigg)^{1.5n-2.5}\gamma_{max}^{3mn-7m}\bigg)
% %     \end{equation*}
% % For the second case. we use similar method to estimate and obtain
% % \begin{align*}
% %     \bfa P(E_{i,j}\cap E_{k,l})&=\bfa P(\ca A^m_{i,l}=\ca A^m_{i,k}=\ca A^m_{j,k}=\ca A^m_{j,l})\cdot\prod_{o\in[n]\setminus\{i,j,k,l\}}\bfa P(\ca A^m_{i,o}=\ca A^m_{j,o}=\ca A^m_{k,o}=\ca A^m_{l,o})\\
% %     &=\bigg(\sum_{\bfa X\in\bb X(\ca A^m_{i,l}=\ca A^m_{i,k}=\ca A^m_{j,k}=\ca A^m_{j,l})}\prod_{c\in[m]}\ff{i,l}\ff{i,k}\\
% %     &\ff{j,k}\ff{j,l}\bigg)\\
% %     &\cdot\bigg(\prod_{o\in[n]\setminus\{i,j,k,l\}}\sum_{\bfa X\in\bb X(\ca A^m_{i,o}=\ca A^m_{j,o}=\ca A^m_{k,o}=\ca A^m_{l,o})}\prod_{c\in[m]}\ff{i,o}\\
% %     &\ff{j,o}\ff{k,o}\ff{l,o}\bigg)\\
% %     &=O\bigg(\bigg(\frac{4^m}{\sqrt m}\bigg)^{2n-6}\gamma_{max}^{4m+4m(n-4)}\bigg)
% % \end{align*}
% % Hence the $\gamma_n$ can be estimated by:
% % \begin{equation*}
% % \gamma_n=O\bigg(\binom{n}{3}\bigg(\frac{4^m}{\sqrt m}\bigg)^{1.5n-2.5}\gamma_{max}^{3mn-7m}+\binom{n}{4}\bigg(\frac{4^m}{\sqrt m}\bigg)^{2n-6}\gamma_{max}^{4mn-12m}  \bigg)
% % \end{equation*}
% % To have that $\gamma_n=O(\mu_n^2)$, we prove the above threshold.
% % \begin{align*}
% %     &\log(\frac{\gamma_{max}}{\gamma_{min}})=\Omega\bigg(\max\bigg\{\frac{2m\log 2-\log m +12m\log\gamma_{max}}{4nm},\frac{m\log2-0.25\log n+m\log\gamma_{min}}{3m}\bigg\}\bigg)
% % \end{align*}
% % % For the converse, using the first moment method we have
% % % \begin{equation*}
% % %     \mu_n=O\bigg(n^2\bigg(\frac{4^m}{\sqrt m}\bigg)^{n-2}\gamma_{max}^{2mn}\bigg)\rightarrow 0
% % % \end{equation*}
% % % or
% % % \begin{equation*}
% % %   \log\frac{1}{\gamma_{max}}=\Omega\bigg(\frac{\log n}{mn}+\log 2 -\frac{\log m}{4m}\bigg)
% % % \end{equation*}
% % % Then the automorphism will asymptotically exist.

% % \end{proof}


% % \begin{proof}
% % The proof of this lemma comes directly from the definition exact ranking. To guarantee exact ranking, MAP can only have $o(1)$ probability of error.
% % \end{proof}
% % Here we introduce a general definition of automorphism on weighted directed graphs


% % The above fact can be further relaxed to the following one:
% % \begin{lemma}\label{lm:3}
% % Let $\ca A^m(i,j)$ be the matrix that satisfies the following:
% % \begin{equation*}
% %     \ca A^m(i,j)_{k,l}=\left\{\begin{matrix}
% %  \ca A^m_{k,l}  &\text{ if } (k,l)\neq(i,j)\\
% %   0& \text{ if }(k,l)=(j,i) \\
% %   0&\text{ otherwise }
% % \end{matrix}\right.
% % \end{equation*}
% % Then the weighted directed graph induced by $\ca A^m(i,j)$ cannot be exactly ranked with MAP estimator if there exists an $\ca A^m(i,j)$m $i\leq j\wedge i,j\in[n]$ with $\Theta (1)$ probability.
% % \end{lemma}
% % \begin{proof}
% % We note that MAP will fail with $\Theta(1)$ probability on $\ca A^m(i,j)$
% % \end{proof}
% % The following lemma provides a general version of the above arguments.


% % \begin{fact}[Transitivity]
% % When $(i,j)$ and $(j,k)$ are indistinguishable pairs, $(i,k)$ is also an indistinguishable pair.
% % \end{fact}
% Our methodology is based on the following theorem.
% \begin{theorem}\label{thm:5}[Paley-Zygmund inequality] Let $X$ be a non-negative random variable. For all $0<\theta<1$,
% \begin{equation*}
%     \bfa P[X\geq\bb EX]\geq(1-\theta)^2\frac{(\bb EX)^2}{\bb E[X^2]}
% \end{equation*}
% \end{theorem}
% Taking $\theta\rightarrow 0$, the above theorem directly leads to
% \begin{corollary}\label{cor:3.1}Let $X$ be a non-negative random variable. Then
% \begin{equation*}
%     \bfa P(X>0)\geq\frac{(\bb EX)^2}{\bb E[X^2]}
% \end{equation*}
% \end{corollary}
% Then the following corollary comes directly from corollary~\ref{cor:3.1}
% \begin{corollary}
% Let $B_n=E_{1}\cup \cdots\cup E_{m(n)}$. where $E_{1},...,E_{m(n)}$ is a collection of events for each $n$. Write $i\overset{n}{\sim} j $ if $i\neq j$ and $E_{i}$ and $E_{j}$ are not independent. Then, letting
% \begin{equation*}
%     \mu_n:=\sum_{i=1}^{m(n)}\bfa P(E_{i}),\;\;\;\;\gamma_n:=\sum_{i\overset{n}{\sim}j}\bfa P(E_{i}\cap E_{j})
% \end{equation*}
% \label{cor1.2}
% where the second sum is over ordered pairs, we have $\lim_{n\rightarrow\infty}\bfa P(B_n)>0$ whenever $\mu_n\rightarrow\infty$ and $\gamma_n\leq C\mu_n^2$ for some $C>0$. If moreover $\gamma_n=o(\mu_n^2)$ then $\lim_{n\rightarrow\infty}\bfa P(B_n)=1$.
% \end{corollary}
% \begin{proof}
% Take $X:=X_n=\sum_{i=1}^{m(n)}\bfa 1_{E_i}$ in the previous theorem. We note that
% \begin{equation*}
%     Var[X_n]=\sum_{i}Var[\bfa 1_{E_i}]+\sum_{i\neq j}Cov[\bfa 1_{E_i},\bfa 1_{E_j}]
% \end{equation*}
% where we have
% \begin{equation*}
%     Var[\bfa 1_{E_i}]=\bb E[(\bfa 1_{E_i})^2]-(\bb E[\bfa 1_{E_i}])^2\leq\bfa P(E_i)
% \end{equation*}
% and, if $E_i$ and $E_j$ are independent,
% \begin{equation*}
%     Cov[\bfa 1_{E_i},\bfa 1_{E_j}]=0
% \end{equation*}
% whereas, if $i\overset{n}{\sim} j$,
% \begin{equation*}
%     Cov[\bfa 1_{E_i},\bfa 1_{E_j}]=\bb E[\bfa 1_{E_i}\bfa 1_{E_j}]-\bb E[\bfa 1_{E_i}]\bb E[\bfa 1_{E_j}]\leq\bfa P[E_i\cap E_j]
% \end{equation*}
% Hence,
% \begin{equation*}
%     \frac{Var[X_n]}{(\bb E X_n)^2}\leq\frac{\mu_n+\gamma_n}{\mu_n^2}=\frac{1}{\mu_n}+\frac{\gamma_n}{\mu_n^2}
% \end{equation*}
% and we note that
% \begin{equation*}
%     \frac{(\bb EX_n)^2}{E[X_n^2]}=\frac{(\bb EX_n)^2}{(\bb EX_n)^2+Var[X_n]}=\frac{1}{1+ \frac{Var[X_n]}{(\bb E X_n)^2}}
% \end{equation*}
% Applying the previous corollary yield the final result.
% \end{proof}

\subsubsection{Impossibility}

In this section, we denote $F_{i,j}$ as the event that $\bfa A_{i,k}^m>\bfa A_{j,k}^m$ for $k\in[n]\setminus\{i,j\}$ and denote $\bfa P_{i,j}=\bfa P(F_{i,j})$. Let $\bfa A\in\{0,1\}^{n\times n}$ denote the set of random variables in the state space where $\bfa A_{i,j}^m$ represents number of victory of party $i$ over $j$, when the number of comparisions toted $m$. In particular, we let $\bfa A_{i,i}=0$ for all $i\in[n]$, then the following lemma gives a necessary condition on exact ranking, connecting it to the standard hypothesis testing problem.

We first state a sufficient condition of impossibility.
\begin{lemma}\label{lm1}
For a pair of vertices $(i,j)$ with $i>j$, if $\bfa P(\bigcup_{i<j,i,j\in[n]}F_{i,j})=\Theta (1)$, then the Bayes estimator will fail the exact ranking.
\end{lemma}
% \begin{remark}
% Lemma 1 is a straight forward argument. In particular, if 
% \end{remark}
We then gave the Chernoff bound for the Binomial random variables.
\begin{lemma}\label{lm2}
For a binomial $X\sim Binom(n,p)$, when $k\leq np$, the tail inequality is given by Chernoff bound
\begin{align*}
    \bfa P(X\leq k)&=(n-k)\binom{n}{k}\int_{0}^{1-p}t^{n-k-1}(1-t)^kdt\leq\exp\bigg(-nD_{kl}\big(\frac{k}{m}\Vert p\big)\bigg)\\
    &\leq \exp(-2m\big(p-\frac{k}{m}\big)^2)
\end{align*}
\end{lemma}
Then we gave a lower bound on the difference between two binomials, stated by the following lemma
% \begin{proof}
% We define:
% \begin{align*}
%     V(m,p,q,x,y)=\binom{m}{x+y}\binom{m}{x}p^{x}q^{x+y}(1-p)^{m-x}(1-q)^{m-x-y}
% \end{align*}
% Then we have
% \begin{align*}
%     \log(V(m,p,q,x,y))&=\log\binom{m}{x+y}+\log\binom{m}{x}\\
%     &+x\log p+y\log q+(m-x)\log(1-p)+(m-x-y)\log(1-q)
% \end{align*}
% Then we use that for $k\leq N$
% \begin{align*}
%     \log\binom{N}{k}&\geq k\log N-\log k!-\log 4\\
%     \log k!&\leq(k+1)\log((k+1)/e)
% \end{align*}
% which gives
% \begin{align*}
%     \log\binom{N}{k}\geq k\log N-(k+1)\log(k+1)+k-\log 4
% \end{align*}
% and we have
% \begin{align*}
%     \log\binom{m}{x+y}&\geq (x+y)\log m-(x+y+1)\log (x+y+1)+x+y-\log 4\\
%     \log\binom{m}{x}&\geq x\log m-(x+1)\log(x+1)+x-\log 4
% \end{align*}
% Combining pieces, the following hold
% \begin{align*}
%      \log(V(m,p,q,x,y))&\geq (x+y)\log m+x\log m+ (m-x)\log(1-p)+(m-x-y)\log(1-q)\\
%                       &-(x+y+1)\log(x+y+1)-(x+1)\log(x+1)+x\log p+y\log q\\
%                       &+2x+y
% \end{align*}
% maximizing over $x,y$ we see that:
% \begin{align*}
%     \log\bfa P(X\geq Y)\geq \max_{x,y}\log (V(m,p,q,x,y))\geq
% \end{align*}
% \end{proof}
Then we review the Berry-Esseen theorem~\citep{berry1941accuracy}, which establishes the asymptotic rate of large deviation.
\begin{theorem}[Berry-Esseen]
Let $X_1,\ldots,X_n$ be independent random variables with the same distribution such that $
    \bb EX_j=0,\;\;\bb EX_j^2=\sigma^2>0,\;\;\bb E|X_j|^3<\infty$, Let $\rho=\frac{\bb E|X_j|^3}{\sigma^3}$ and
    \begin{equation*}
        \Phi(x)=\frac{1}{\sqrt{2\pi}}\int_{-\infty}^xe^{\frac{t^2}{2}}dt
    \end{equation*}
then, for any $n$, we have
\begin{align*}
    \sup_{x}\bigg|\bfa P\bigg\{\frac{1}{\sigma\sqrt{n}}\sum_{j=1}^nX_j\leq x\bigg\}-\Phi(x)\bigg|\leq A\frac{\rho}{\sqrt{n}}
\end{align*} 
where $A\leq 0.7655$ is the absolute positive constant.
\end{theorem}
% \begin{definition}[Stochastic domination]
% Let $\mu$ and $\nu$ be probability measures on $\bb R$. The measure $\mu$ is said to stochastically dominate $\mu$, denote by $\mu\succeq\nu$, if for all $x\in\bb R$
% \begin{equation*}
%     \mu[(x,+\infty)]\geq\nu[(x,+\infty)]
% \end{equation*}
% A real random variable $X$ stochastically dominates $Y$, denoted by $X\succeq Y$, if the law of $X$ dominates the law of $Y$.
% \end{definition}
% \begin{lemma}[Binomial is dominated by Poisson]
% When $\lambda\geq-\log(1-p)$, $Poi(m\lambda)$ stochastic-ally dominates $Binom(m,p)$
% \end{lemma}
The following lemma is a direct application of Berry-Esseen theorem.
\begin{lemma}\label{lm4}
Given a binomial $X\sim Binom(m,p)$, its c.d.f. can be estimated by:
\begin{align*}
    \sup_{x}\bigg|\bfa P(\bfa X\leq x)-\Phi(x)\bigg|\leq\frac{C_1}{\sqrt m}
\end{align*}
its p.d.f. can be estimated by
\begin{align*}
    \sup_x\bigg|\bfa P(\bfa X=x)-\frac{1}{\sqrt{2\pi p(1-p)m}}\exp\bigg(-\frac{(x-mp)^2}{p(1-p)m}\bigg)\bigg |\leq\frac{C_2}{\sqrt{m}}
\end{align*}
for some universal constant $C_1,C_2$ and $x\in\bb N$
\end{lemma}
By Berry-Esseen theorem and use the fact that Binomial random variables $\bfa X\sim Binom(m,p)$ can be seen as the ensemble of Bernoulli random variables $\bfa X=\sum_{i=1}^m\bfa x_i$ with $\bfa x_i\sim Bern(p)$ for all $i\in[m]$.
\begin{align*}
    \sup_{x}\bigg|\bfa P\bigg (\frac{1}{\sqrt{p(1-p)m}}(\bfa X-mp)\leq x\bigg )-\Phi (x)\bigg |\leq \frac{C_1}{\sqrt m}
\end{align*}
Or
\begin{align*}
    \sup_x\bigg|\bfa P(\bfa X\leq x)-\Phi\bigg (\frac{x-mp}{\sqrt{p(1-p)m}}\bigg )\bigg|\leq\frac{C_1}{\sqrt{m}}
\end{align*}
And we also have that for all $x\in\bb N$:
\begin{align*}
    &\bigg|\bfa P(\bfa X\leq x)-\bfa P(\bfa X\leq x-1)-\bigg(\Phi\bigg (\frac{x-mp}{\sqrt{p(1-p)m}}\bigg)-\Phi\bigg(\frac{x-1-mp}{\sqrt{p(1-p)m}}\bigg)\bigg)\bigg|\\
    &=\bigg | \bfa P(\bfa X=x)-\frac{1}{\sqrt{2\pi p(1-p)m}}\exp\bigg (-\frac{(x-mp)^2}{p(1-p)m}\bigg)\bigg |\leq\frac{C_2}{\sqrt{m}}
\end{align*}
where we already used the fact that
\begin{equation*}
    \frac{1}{\sqrt{2\pi p(1-p)m}}\bigg [\exp\bigg(-\frac{(x-mp)^2}{p(1-p)m}\bigg)-\exp\bigg(-\frac{(x-1-mp)^2}{p(1-p)m}\bigg)\bigg]\leq\frac{C_3}{\sqrt m}
\end{equation*}
% \begin{lemma}[Hoeffding's Bound on the difference between binomials]
% Given two random variables $X\sim Binom(m,p_1)$, $Y\sim Binom(m,p_2)$ Then the following holds for their difference:
% \begin{equation*}
%     \bfa P(X\leq Y)\leq\exp\bigg(-2\bigg(\frac{p_2(1-p_1)}{p_1(1-p_2)+p_2(1-p_1)} - \frac 12\bigg)^2 \big(p_1(1-p_2) + p_2(1-p_1)\big) m\bigg)
% \end{equation*}
% \end{lemma}
Then we review the Paley-Zygmund inequality, which is stated as
\begin{lemma}[Paley-Zygmund]
For random variable $Z>0$, for $\theta\in(0,1)$ we have
\begin{align*}
    \bfa P(Z\geq\theta\bb E[Z])\geq(1-\theta)^2\frac{\bb E[Z]^2}{\bb E[Z^2]}
\end{align*}
And for general random variable, we have
\begin{align*}
    \bfa P(\exp(tZ)\geq\theta\bb E[\exp(tZ)])\geq(1-\theta)^2\frac{\bb E[\exp(tZ)]^2}{\bb E[\exp(2tZ)]}
\end{align*}
\end{lemma}


which directly implies
\begin{corollary}[Second Order Method]
$
\bfa P(Z\geq 0)\geq\frac{\bb E[Z]^2}{\bb E[Z^2]}
$
\end{corollary}
and further implies
\begin{corollary}
Let $B_n=E_{1}\cup \cdots\cup E_{m(n)}$. where $E_{1},...,E_{m(n)}$ is a collection of events for each $n$. Write $i\overset{n}{\sim} j $ if $i\neq j$ and $E_{i}$ and $E_{j}$ are not independent. Then, letting
\begin{equation*}
    \mu_n:=\sum_{i=1}^{m(n)}\bfa P(E_{i}),\;\;\;\;\gamma_n:=\sum_{i\overset{n}{\sim}j}\bfa P(E_{i}\cap E_{j})
\end{equation*}
\label{cor1.2}
where the second sum is over ordered pairs, we have $\lim_{n\rightarrow\infty}\bfa P(B_n)>0$ whenever $\mu_n\rightarrow\infty$ and $\gamma_n\leq C\mu_n^2$ for some $C>0$. If moreover $\gamma_n=o(\mu_n^2)$ then $\lim_{n\rightarrow\infty}\bfa P(B_n)=1$.
\end{corollary}
\begin{proof}
Take $X:=X_n=\sum_{i=1}^{m(n)}\bfa 1_{E_i}$ in the previous theorem. We note that
\begin{equation*}
    Var[X_n]=\sum_{i}Var[\bfa 1_{E_i}]+\sum_{i\neq j}Cov[\bfa 1_{E_i},\bfa 1_{E_j}]
\end{equation*}
where we have
\begin{equation*}
    Var[\bfa 1_{E_i}]=\bb E[(\bfa 1_{E_i})^2]-(\bb E[\bfa 1_{E_i}])^2\leq\bfa P(E_i)
\end{equation*}
and, if $E_i$ and $E_j$ are independent,
\begin{equation*}
    Cov[\bfa 1_{E_i},\bfa 1_{E_j}]=0
\end{equation*}
whereas, if $i\overset{n}{\sim} j$,
\begin{equation*}
    Cov[\bfa 1_{E_i},\bfa 1_{E_j}]=\bb E[\bfa 1_{E_i}\bfa 1_{E_j}]-\bb E[\bfa 1_{E_i}]\bb E[\bfa 1_{E_j}]\leq\bfa P[E_i\cap E_j]
\end{equation*}
Hence,
\begin{equation*}
    \frac{Var[X_n]}{(\bb E X_n)^2}\leq\frac{\mu_n+\gamma_n}{\mu_n^2}=\frac{1}{\mu_n}+\frac{\gamma_n}{\mu_n^2}
\end{equation*}
and we note that
\begin{equation*}
    \frac{(\bb EX_n)^2}{E[X_n^2]}=\frac{(\bb EX_n)^2}{(\bb EX_n)^2+Var[X_n]}=\frac{1}{1+ \frac{Var[X_n]}{(\bb E X_n)^2}}
\end{equation*}
Applying the previous corollary yield the final result.
\end{proof}
We have the following several technical lemmas
\begin{lemma}
Let $X\sim Binom(m,p)$ and $Y\sim Binom (m,q)$ with $p<q$ and suppose $m$ is large enough, we have 
\begin{align*}
    \bfa P(X\geq Y)=1-\Phi(x)\geq\bigg (\frac{x}{x^2+1}\bigg )\frac{1}{\sqrt{2\pi}}\exp(-\frac{x^2}{2}) 
\end{align*}
with $x=\sqrt{\frac{m(q-p)^2}{p(1-p)+q(1-q)}}$
\end{lemma}
\begin{proof}
Denote $\psi_X$ as the moment generating function of random variable $X-\bb E[X]$. By normal approximation, we have
\begin{align*}
    \psi_{X-Y}(t)=\psi_X(t)/\psi_Y(t)=\bigg(\frac{(1-p)e^{-pt}+pe^{(1-p)t}}{(1-q)e^{-qt}+qe^{(1-q)t}}\bigg)^m\rightarrow\exp\bigg(\frac{(p(1-p)-q(1-q))nt^2}{2}\bigg)
\end{align*}
Then we use the fact that $X-Y\sim N(m(p-q),m(p(1-p)+q(1-q)))=N(\mu(p,q),\sigma^2(p,q))$ and obtain that:
\begin{align*}
     \bfa P(X\geq Y)&=\bfa P(X-Y\geq 0)=1-\Phi\bigg(\sqrt{\frac{-m(p-q)^2}{p(1-p)+q(1-q)}}\bigg)+O(\frac{1}{\sqrt m})
\end{align*}
where $\Phi(x)=\frac{1}{\sqrt{2\pi}}\int_{-\infty}^x e^{-\frac{t^2}{2}}dt$ is the c.d.f. of standard normal distribution. The extra term error is given by Berry-Esseen theorem. Then we recall the lowerbound on the Gaussian tail that for all $x>0$, the following holds
\begin{align*}
    1-\Phi(x)\geq\frac{x}{x^2+1}\frac{1}{\sqrt{2\pi}}e^{-\frac{x^2}{2}}
\end{align*}
with the assumption that $m$ is very large, we finish the proof.
\end{proof} 

% \begin{lemma}\label{lm:88}
% Given two random variables $X\sim Binom(m,p_1)$, $Y\sim Binom(m,p_2)$. Assuming $p_1\geq p_2$, then the following holds:
% \begin{equation*}
%     \bb E[(Y-X)^2]\leq  m (p_1-p_2)+m(m-1)(p_1-p_2)^2
% \end{equation*}
% \end{lemma}
% \begin{proof}
% We denote $Y-X=\sum_{i=1}^m\sigma_m$ by a sum of $m$ random variables i.i.d. $\sigma_1$ induces the following probability measure:
% \begin{align*}
%   \sigma_1= \left\{\begin{array}{ll}
% 1 &\text{ with probability } p_2(1-p_1)  \\
% 0 &\text{ with probability } p_2p_1+(1-p_2)(1-p_1)  \\
% -1&\text{ with probability } p_1(1-p_2)\\
% \end{array}\right.
% \end{align*}
% And the moment generating function, when $\lambda\geq 0$, is given by 
% \begin{align*}
%     \phi_{\sigma}(\lambda)=\bb E[\exp(\lambda(\sigma))]&=p_2(1-p_1)\exp(\lambda)+p_1p_2+(1-p_2)(1-p_1)+p_1(1-p_2)\exp(-\lambda)\\&\leq\exp(-\lambda\bb E[\sigma]+\frac{1}{2}\lambda^2\zeta^2)
% \end{align*}
% By Taylor expansion until the second order, we obtain that
% \begin{equation*}
%     \bb E[\sigma]=p_1-p_2\;\;\zeta=\sqrt{(-2p_1p_2+p_1+p_2)-(p_1-p_2)^2}
% \end{equation*}
% Therefore the generative function of $Y-X$ can be bounded by:
% \begin{align*}
%     \phi_{Y-X}(\lambda)&=\bb E[\exp(\lambda(Y-X)]\\
%     &=\prod_{i=1}^m\bb E[\exp(\lambda\sigma_i)]\\
%     &=\sum_{i=1}^\infty\bb E[\sigma^i]\frac{\lambda^i}{i!}\\
%     &\leq\exp(-m\lambda\bb E[\sigma]+\frac{m}{2}\lambda^2\zeta^2)\\
%     &=\sum_{i=1}^\infty\frac{-\lambda^im^i\bb E[\sigma]^i}{i!}+\sum_{i=1}^\infty\frac{m^{i}\lambda^{2i}}{2^i(i)!}\zeta^{2i}
% \end{align*}
% Hence, by comparing the term on the r.h.s. and l.h.s., we can see that:
% \begin{equation*}
%     \bb E[(Y-X)^2]=m^2\bb E[\sigma]^2 +m\zeta^2\leq m (p_1+p_2-p_1p_2)+m(m-1)(p_1-p_2)^2
% \end{equation*}
% \end{proof}

\begin{lemma}
\label{lm10}
Let $\bfa X\sim Binom(m,p_1),\bfa Y\sim Binom(m,p_2),\bfa Z\sim Binom(m,p_3)$. Assuming $p_1<p_2<p_3$ and $m$ is large, then 
\begin{align*}
    \bfa P(\bfa X>\max\{\bfa Y,\bfa Z\})&\leq(1+8p_1(1-p_1))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)+\frac{(-1-2p_3-2p_2)^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)
\end{align*} 
\end{lemma}
\begin{proof}
Using lemma \ref{lm2} and \ref{lm4}, we divide the range $\{1,\ldots,m\}$ into $\{1,\ldots,\lfloor\min\{p_2,p_3\}\rfloor\}$, $\{\lfloor\min\{p_2,p_3\}\rfloor+1,\ldots,\lfloor\max\{p_2,p_3\}\rfloor\}$, and $\{\lfloor\max\{p_2,p_3\}\rfloor+1,\ldots,m\}$ and upper bound them separately.
Also, using the normal approximation and Berry Esseen, when $y\leq mp_2$ and $z\leq mp_3$, the following holds.
\begin{align*}
    \bfa P(\bfa Y\leq y)&\leq \exp\bigg (-\frac{(y-mp_2)^2}{2mp_2(1-p_2)}\bigg)+O(\frac{1}{\sqrt m})\\
    \bfa P(\bfa Z\leq z)&\leq\exp\bigg(-\frac{(z-mp_3)^2}{2mp_3(1-p_3)}\bigg)+O(\frac{1}{\sqrt m})
\end{align*}
which implies the following
\begin{align*}
    \bfa P(\bfa X>\bfa Y,\bfa X>\bfa Z)&=\int_{-\infty}^\infty \bfa P(\bfa X=x)\bfa P(\bfa Y<x)\bfa P(\bfa Z<x)dx\\
    &=\sum_{i=1}^m\bigg[\bigg(\sum_{j=1}^{i-1}\binom{m}{j}p_2^j(1-p_2)^{m-j}\bigg)\bigg(\sum_{k=1}^{i-1}\binom{m}{j}p_3^k(1-p_3)^{m-k}\bigg)\bigg]\binom{m}{i}p_1^i(1-p_1)^{m-i}\\
    &\leq\sum_{i=1}^{m\lfloor\min(p_2,p_3)\rfloor}\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-\frac{(i-mp_2)^2}{2mp_2(1-p_2)}-\frac{(i-mp_3)^2}{2mp_3(1-p_3)}\bigg)\\
    &+\sum_{i=\lceil m\min(p_3,p_2)\rceil}^{m\lfloor m\max(p_2,p_3)\rfloor}\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-\frac{(i-m\max\{ p_2,p_3\})^2}{2m\max\{p_2,p_3\}(1-\max\{p_2,p_3\})}\bigg)\\
    &+\sum_{i=\lfloor m\max\{p_2,p_3\}\rfloor}^m\binom{m}{i}p_1^i(1-p_1)^{m-i}\\
    &\leq\sum_{i=1}^{m\lfloor\min(p_2,p_3)\rfloor}\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-\frac{(i-mp_2)^2}{2mp_2(1-p_2)}-\frac{(i-mp_3)^2}{2mp_3(1-p_3)}\bigg)\\
    &+\sum_{i=\lfloor m\min(p_3,p_2)\rfloor}^m\binom{m}{i}p_1^i(1-p_1)^{m-i}
    \end{align*}
    where the last inequality comes from the fact that when $i\in\{\lfloor\min\{(p_2,p_3)\}\rfloor+1,\ldots,\lfloor\max\{(p_2,p_3)\}\rfloor\}$
    \begin{align*}
        \exp\bigg(-\frac{(y-m\max(p_2,p_3))^2}{2m\max\{p_2,p_3\}(1-\max\{p_2,p_3\})}\bigg)\leq 1
    \end{align*}
    We upperbound the $2$ terms seperately. Since we have $\min(p_2,p_3)>p_1$ the upperbound to the second term can be directly obtained by the Hoeffding's inequality, given by:
    \begin{align*}
        \sum_{i=\lfloor m\min(p_3,p_2)\rfloor}^m\binom{m}{i}p_1^i(1-p_1)^{m-i}&=\bfa P(\bfa X>\lfloor m\min(p_3,p_2)\rfloor)\\
        &\leq\exp(-\frac{(mp_1-m\lfloor\min(p_3,p_2)\rfloor)^2}{2mp_1(1-p_1)})+O(\frac{1}{\sqrt m})
    \end{align*}
    To upperbound the first term, we have
    \begin{align*}
    &\sum_{i=1}^{m\lfloor\min(p_2,p_3)\rfloor}\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-\frac{(i-mp_2)^2}{2mp_2(1-p_2)}-\frac{(i-mp_3)^2}{2mp_3(1-p_3)}\bigg)\\
    % &\leq\sum_{i=1}^{m\lfloor\min(p_2,p_3)\rfloor}\frac{m^i\log^i(1-p_1)}{i!}\exp\bigg(-m\bigg(\log(1-p_1)+2\big((p_3-\frac{i}{m})^2+(p_2-\frac{i}{m})^2\big)\bigg)\bigg)\\
    % &\leq \int_{0}^{m\lfloor\min(p_2,p_3)\rfloor}\frac{1}{\sqrt{2\pi mp_1(1-p_1)}}\exp\bigg(-\frac{(x-mp_1)^2}{2mp_1(1-p_1)}-2m\big((p_3-\frac{x}{m})^2+(p_2-\frac{x}{m})^2\big)\bigg)dx+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &\leq \int_{0}^{m\lfloor\min(p_2,p_3)\rfloor}\frac{1}{\sqrt{2\pi mp_1(1-p_1)}}\exp\bigg(-\frac{(x-mp_1)^2}{2mp_1}-\frac{(x-mp_2)^2}{2mp_2(1-p_2)}-\frac{(x-mp_3)^2}{2mp_3(1-p_3)}\bigg)dx\\
    &+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &=\int_{0}^{m\lfloor\min(p_2,p_3)\rfloor}(2\pi mp_1(1-p_1))^\frac{-1}{2}\exp-\bigg(\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}x^2+(-1-2p_3-2p_2)x+m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)\bigg)dx\\
    &+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &=( mp_1(1-p_1))^{-\frac{1}{2}}\exp-\bigg(m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)-\frac{(-1-2p_3-2p_2)^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &\int_{0}^{m\lfloor\min(p_2,p_3)\rfloor}\frac{1}{\sqrt{2\pi}}\exp-\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}\bigg(x+\frac{-1-2p_3-2p_2}{2\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)^2dx+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &= (1+8p_1(1-p_1))^{-\frac{1}{2}}\exp-\bigg(m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)-\frac{(-1-2p_3-2p_2)^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)\\
    &(\Phi(A(m))-\Phi(B(m)))+O(\frac{\exp(-Cm^2)}{\sqrt{m}})\\
    &\leq(1+8p_1(1-p_1))^{-\frac{1}{2}}\exp-\bigg(m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)-\frac{(-1-2p_3-2p_2)^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)+O(\frac{\exp(-Cm^2)}{\sqrt{m}})
    \end{align*}
    where $\Phi(x)=\bfa P(X\leq x)$ where $X\sim N(0,1)$ and we immediately have
    \begin{align*}
        \Phi(x_1)-\Phi(x_2)\leq 1
    \end{align*}
    which completes the estimate.
%     &\leq \int_{0}^m(2\pi mp_1)^{-\frac{1}{2}}\bigg(\frac{(x-mp_1)^2}{2mp_1}+2m\big((p_3-\frac{x}{m})^2+(p_2-\frac{x}{m})^2\big)\bigg)^{-1}dx\\
%     &=\int_{0}^m(2\pi mp_1)^{-\frac{1}{2}}\bigg(\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}x^2+(-1-2p_3-2p_2)x+m(\frac{1}{2}p_1^2+2p_2^2+2p_3^2)\bigg)
% \end{align*}
% We know that when $ax^2+bx+c>0$ for all $x$ $(4ac-b^2>0)$, the integral yield the following:
% \begin{equation*}
%     \int \frac{1}{ax^2+bx+c}dx=\frac{1}{\sqrt{b^2-4ac}}\ln\bigg|\frac{2ax+b-\sqrt{b^2-4ac}}{2ax+b+\sqrt{b^2+4ac}}\bigg|+k
% \end{equation*}
\end{proof}
\begin{lemma}\label{lm11}
Let $\bfa X\sim Binom(m,p_1),\bfa Y\sim Binom(m,p_2),\bfa Z\sim Binom(m,p_3)$. Assuming $p_1\leq\min(1-p_2,p_3)$ then  \begin{align*}
    \bfa P(\bfa Y>\bfa X>\bfa Z)&\leq(1+8p_1(1-p_1))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}p_1^2+2(1-p_2)^2+2p_3^2)\\
    &+\frac{(-1-2p_3-2(1-p_2))^2}{4\frac{1+8p_1(1-p_1)}{2mp_1(1-p_1)}}\bigg)
\end{align*}when $m$ is large but not necessarily going to infinity.
\end{lemma}
\begin{proof}
Similar to the proof of lemma \ref{lm10}, we start by writing it as an integral. In particular, we observed that by replacing $p_2$ in Lemma \ref{lm10} by $1-p_2$, we will obtain the proof. The details is stated by
\begin{align*}
\bfa P(\bfa Y>\bfa X>\bfa Z)&=\int_{-\infty}^\infty\bfa P(\bfa Y >x)\bfa P(\bfa X=x)\bfa P(
\bfa Z<x)dx\\
&=\sum_{i=1}^m\bigg[\bigg(\sum_{j=i}^m\binom{m}{j}p_2^j(1-p_2)^{m-j}\bigg)\bigg(\sum_{k=1}^{i-1}\binom{m}{j}p_3^k(1-p_3)^{m-k}\bigg)\bigg]\binom{m}{i}p_1^i(1-p_1)^{m-i}
% &\leq\sum_{i=1}^m\binom{m}{i}p_1^i(1-p_1)^{m-i}\exp\bigg(-2m\big ((p_2-\frac{m-i}{m})^2+(p_2-\frac{i}{m})^2\big )\bigg)\\
% &\leq\int_{0}^m\frac{1}{\sqrt{2\pi mp_1}}\exp\bigg(-\frac{(x-mp_1)^2}{2mp_1}-2m\big ((p_2-\frac{m-i}{m})^2+(p_2-\frac{i}{m})^2\big )\bigg)dx\\
% &=(2\pi m p_1)^{-\frac{1}{2}}\int_{0}^m\exp\bigg(-\frac{(x-mp_1)^2}{2mp_1}-2m\big((p_2-\frac{m-i}{m})^2+(p_2-\frac{i}{m})^2\big)\bigg)dx\\
% &\leq(4p_1+1)^{-\frac{1}{2}}\exp-\bigg(m(\frac{1}{2}p_1^2+2(1-p_2)^2+2p_3^2)-\frac{-1-2p_3-2(1-p_2))^2}{2\frac{4p_1+1}{mp_1}}\bigg)
\end{align*}
where the argument follows exactly from the previous lemma.
\end{proof}
% For the joint event over $4$ indices, the following should hold:
% \begin{lemma}
% Let $\bfa X\sim Binom(m,p_1)$, $\bfa Y\sim Binom(m,p_2)$, $\bfa Z\sim Binom(m,p_3)$ and $\bfa W\sim Binom(m,p_4)$ and independent. Assume that $p_1<\min(p_2,p_3)<\max(p_2,p_3)<p_4$ and $m$ is large, then $\bfa P(\bfa X>\min(\bfa Y,\bfa Z)\geq\max(\bfa Y,\bfa Z)>\bfa W)$ 
% \end{lemma}
% \begin{proof}
% We adopt similar method as proving the previous two lemmas. We cannot directly use tailbound but use the fact that $Binom(m,p)$ is dominated by $\ca N(mp,mp)$ when $m$ is very large.
% \begin{align*}
%     &\bfa P(\bfa X>\max(\bfa Y,\bfa Z)\geq\min(\bfa Y,\bfa Z)>\bfa W)\\
%     &=\sum_{i=2}^{m}\binom{m}{i}p_1^i(1-p_1)^{m-i}\sum_{l=i-2}^{m-2}\binom{m}{l}p_4^i(1-p_4)^{m-i}\bigg(\sum_{j=i+1}^{l-1}\binom{m}{j}p_2^l(1-p_2)^{m-l}\bigg)\\
%     &\bigg(\sum_{k=i+1}^{l-1}\binom{m}{k}p_3^k(1-p_3)^{m-k}\bigg)\\
%     &\int_{}
% \end{align*}
% \end{proof}
Then the following theorem gives the impossibility condition according to lemma \ref{lm1}.
\begin{theorem}
Let $\Delta=\sum_{k\in[n]\setminus\{a,b\}}| M_{a,k}-M_{b,k}|$. Assuming that $m$ is sufficiently large. Then the following implies impossibility.
\begin{align*}
    \Delta\leq\sqrt{\frac{\log n}{mn}+\frac{\log(8\gamma_{\min}(1-\gamma_{\min})+1)}{m}+\frac{2K}{n}}
\end{align*}
with 
\begin{align*}
    K&=\inf_{i,j,k}\sum_{o\in[n]\setminus\{i,j,k\}}\bigg(\frac{1}{2}M_{k,o}^2+2M_{j,o}^2+2M_{i,o}^2-\frac{M_{k,o}}{2(8M_{k,o}(1-M_{k,o})+1)}\big(1+2M_{k,o}+2M_{o,i}\big)^2\bigg)\\
    \gamma_{\min}&=\inf_{i,j}M_{i,j}
\end{align*}
\end{theorem}
\begin{proof}
Let $(a,b)=\argmin_{(i,j)}\bfa P_{i,j}$. We then use the independence condition, lemma \ref{lm:88}, note that $\bfa X_{a,k}\sim Binom(m, M_{a,k})$ and $\bfa X_{b,k}\sim Binom(m,M_{b,k})$, by Hoeffding's inequality, we have
\begin{align*}
\bfa P(F_{a,b})&=\prod_{k\in[n]\setminus\{a,b\}}\bfa P(\bfa X_{a,k}>\bfa X_{b,k})\\
&=\prod_{k\in[n]\setminus\{a,b\}}\bfa P\bigg(\bfa X_{b,k}-\bfa X_{a,k}-\bb E[\bfa X_{b,k}-\bfa X_{a,k}]<-\bb E[\bfa X_{b,k}-\bfa X_{a.k}]\bigg)\\
&\geq\prod_{k\in[n]\setminus\{a,b\}}\exp\bigg(-\frac{m(M_{a,k}-M_{b,k})^2}{2}\bigg)\\
&=\exp\bigg(\sum_{k\in[n]\setminus\{a,b\}}-\frac{m(M_{a,k}-M_{b,k})^2}{2}\bigg)
% \leq \prod_{k\in[n]\setminus\{a,b\}}\exp\bigg(-2\bigg(\frac{M_{b,k}(1-M_{a,k})}{M_{a,k}(1-M_{b,k})+M_{b,k}(1-M_{a,k})} - \frac 12\bigg)^2\\& \big(M_{a,k}(1-M_{b,k}) + M_{b,k}(1-M_{a,k})\big) m\bigg)\\
% &\leq\exp\bigg(\frac{\sum_{k=1}^n m(M_{a,k}-M_{b,k})^2}{2}\bigg)
\end{align*}
And we let $x_{i,j,o}=\sqrt{\frac{m(M_{j,o}-M_{i,o})^2}{M_{j,o}(1-M_{j,o})+M_{i,o}(1-M_{i,o})}}$ and have
\begin{align*}
    \mu_n^2&:=\bigg(\sum_{i<j}\bfa P(F_{i,j})\bigg)^2\geq\bigg ( \sum_{i<j}\prod_{o\in[n]\setminus\{i,j\}}\bigg (\frac{1}{x_{i,j,o}}-\frac{1}{x_{i,j,o}^3}\bigg )\exp\bigg (-\frac{x_{i,j,o}^2}{2}\bigg )\bigg )^2
\end{align*}
Then we see the following joint events $F_{i,j}\cap F_{j,k}$ between on $i,j,k$ with $i<j<k$
\begin{equation*}
    \left\{\begin{matrix}
F_{i,j}\cap F_{j,k}: &\bfa X_{i,k}>\bfa X_{j,k} \text{ and }\bfa X_{j,i}>\bfa X_{k,i} \text{ and }\bfa X_{i,o}>\bfa X_{j,o}>\bfa X_{k,o} \text{ for all }o\in[n]\setminus\{i,j,k\}\\
F_{i,k}\cap F_{j,k}: & \bfa X_{i,j}>\bfa X_{k,j}\text{ and } \bfa X_{j,i}>\bfa X_{k,i}\text{ and }\bfa X_{i,o}>\bfa X_{k,o},\bfa X_{j,o}>\bfa X_{k,o} \text{ for all }o\in[n]\setminus\{i,j,k\} \\
\end{matrix}\right.
\end{equation*}
By lemma \ref{lm11}, we get that
\begin{align*}
    &\bfa P\bigg(F_{i,j}\cap F_{j,k}\bigg)=\bfa P\bigg( \bfa X_{i,j}>\bfa X_{i,k}>\bfa X_{j,k}\bigg)\cdot\prod_{o\in [n]\setminus\{i,j,k\}}\bfa P\bigg (\bfa X_{i,o}>\bfa X_{j,o}>\bfa X_{k,o}\bigg )\\
    &\leq (1+8M_{i,k}(1-M_{i,k}))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}M_{i,k}^2+2(1-M_{i,j})^2+2M_{j,k}^2)+\frac{(-1-2M_{j,k}-2(1-M_{i,j}))^2}{4\frac{1+8M_{i,k}(1-M_{i,k})}{2mM_{i,k}}}\bigg)\\
    &\cdot\prod_{o\in[n]\setminus\{i,j,k\}} (1+8M_{j,o}(1-M_{j,o}))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}M_{j,o}^2+2(1-M_{i,o})^2+2M_{k,o}^2)\\&
    +\frac{(-1-2M_{k,o}-2(1-M_{i,o}))^2}{4\frac{8M_{j,o}(1-M_{j,o})+1}{2mM_{j,o}}}\bigg)\\
    &\leq\bigg(\prod_{o\in[n]\setminus\{i,j,k\}}(1+8M_{j,o}(1-M_{j,o}))\bigg)^{-\frac{1}{2}}\exp\bigg(-m\sum_{o\in[n]\setminus\{i,j,k\}}\bigg(\frac{1}{2}M_{j,o}^2+2M_{o,i}^2+2M_{k,o}^2\\
    &-\frac{M_{j,o}}{2(8M_{k,o}(1-M_{k,o})+1)}\big(1+2M_{k,o}+2M_{o,i}\big)^2\bigg)\bigg)
\end{align*}
For the second regime, we can upperbound the probability of joint event with lemma \ref{lm10}. 
\begin{align*}
    &\bfa P(F_{i,k}\cap F_{j,k})=\bfa P(\bfa X_{i,j}>\bfa X_{k,j}\text{ and } \bfa X_{i,j}>\bfa X_{i,k})\cdot\prod_{o\in[n]\setminus\{i,j,k\}}\bfa P(\bfa X_{o,k}>\max(\bfa X_{o,i},\bfa X_{o,j}))\\
     &\leq (1+8M_{i,j}(1-M_{i,j}))^{-\frac{1}{2}}\exp\bigg(-m(\frac{1}{2}M_{i,j}^2+2M_{k,j}^2+2M_{i,k}^2)+\frac{(-1-2M_{k,j}-2M_{i,k})^2}{4\frac{1+8M_{i,j}(1-M_{i,j})}{2mM_{i,j}}}\bigg)\\
    &\cdot\prod_{o\in[n]\setminus\{i,j,k\}} (8M_{k,o}(1-M_{k,o})+1))^{-\frac{1}{2}}\exp\bigg(\bigg(-m(\frac{1}{2}M_{o,k}^2+2M_{o,i}^2+2M_{o,j}^2)\\&
    +\frac{(-1-2M_{k,o}-2(1-M_{i,o}))^2}{4\frac{(8M_{k,o}(1-M_{k,o})+1))}{2mM_{k,o}}}\bigg)+\exp(-2m(M_{o,k}-\lfloor\min(M_{o,j},M_{o,i})\rfloor)^2)\bigg)\\
    &\leq\bigg(\prod_{o\in[n]\setminus\{i,j,k\}}(8M_{k,o}(1-M_{k,o})+1)\bigg)^{-\frac{1}{2}}\exp\bigg(-m\sum_{o\in[n]\setminus\{i,j,k\}}\bigg(\frac{1}{2}M_{k,o}^2+2M_{j,o}^2+2M_{i,o}^2\\
    &-\frac{M_{k,o}}{2(8M_{k,o}(1-M_{k,o})+1)}\big(1+2M_{k,o}+2M_{o,i}\big)^2\bigg)\bigg)
\end{align*}
Where in the last inequality we used the fact that $\exp(-mC)\rightarrow 0$ as $m\rightarrow\infty$ for positive $C$.
Then we also give the joint events induced by $4$ complete discrete indices $i,j,k,l$ with $i<j<k<l$. For simplicity, we omit the duplicate term in $[n]\setminus\{i,j,k,l\}$ and only give the possible relationship between those $4$ indices here.
\begin{equation*}
    \left\{\begin{matrix}
F_{i,j}\cap F_{k,l}: &\bfa X_{i,l}>\bfa X_{j,l}>\bfa X_{j,k}\text{ and }\bfa X_{i,l}>\bfa X_{i,k}>\bfa X_{j,k}\\
F_{i,l}\cap F_{j,k}: & \bfa X_{i,k}>\bfa X_{i,j}>\bfa X_{l,j}\text{ and }\bfa X_{i,k}>\bfa X_{l,k}>\bfa X_{l,j}\\
F_{i,k}\cap F_{j,l}:&\bfa X_{i,l}>\bfa X_{i,j}>\bfa X_{k,j}\text{ and }\bfa X_{i,l}>\bfa X_{k,l}>\bfa X_{k,j}
\end{matrix}\right.
\end{equation*}
Although these events is connecting $4$ indices in the graph, the multiplicity is always $1$ , which implies that they can be ignored. Henceforth, the only term we need to consider is in the following form, where we take the first case as an example
\begin{align*}
    \bfa P(F_{i,j}\cap F_{k,l})&=\bfa P(\bfa X_{i,l}>\max(\bfa X_{j,l},\bfa X_{i,k})>\bfa X_{j,k})\cdot\prod_{o\in[n]\setminus\{i,j,k,l\}}\bfa P(\bfa X_{i,o}<\bfa X_{j,o},\bfa X_{k,o}<\bfa X_{l,o})\\
    &\leq\prod_{o\in[n]\setminus\{i,j,k,l\}}\bfa P(\bfa X_{i,o}<\bfa X_{j,o})\cdot\bfa P(\bfa X_{k,o}<\bfa X_{l,o})=\bfa P(F_{i,j})\cdot\bfa P(F_{k,l})
    \end{align*}
Collecting pieces, we get
\begin{align*}
    \gamma_n&\leq\sum_{i,j,k,l\in[n]}\bfa P(F_{i,j})\cdot\bfa P(F_{k,l})+\sum_{i,j,k\in[n]}\bigg(\prod_{o\in[n]\setminus\{i,j,k\}}(8M_{k,o}(1-M_{k,o})+1)\bigg)^{-\frac{1}{2}}\\
    &\exp\bigg(-m\sum_{o\in[n]\setminus\{i,j,k\}}\bigg(\frac{1}{2}M_{k,o}^2+2M_{j,o}^2+2M_{i,o}^2-\frac{M_{k,o}}{2(8M_{k,o}(1-M_{k,o})+1)}\big(1+2M_{k,o}+2M_{o,i}\big)^2\bigg)\bigg)
    % \\
    % &\leq\sum_{i,j,k,l\in[n]}\bfa P(F_{i,j})\cdot\bfa P(F_{k,l})+\sum_{i,j,k\in[n]}\bigg(\prod_{o\in[n]\setminus\{i,j,k\}}(8M_{k,o}(1-M_{k,o})+1)\bigg)^{-\frac{1}{2}}\\
    % &\exp\bigg(-m\sum_{o\in[n]\setminus\{i,j,k\}}\bigg)
\end{align*}
Note that by corollary~\ref{cor1.2}, we have
\begin{align*}
    \bfa P\bigg (\bigcup_{i<j}F_{i,j}\bigg )\geq\frac{1}{1+\frac{1}{\mu_n}+\frac{\gamma_n}{\mu_n^2}}
\end{align*}$\sum_{i,j,k,l\in[n]}\bfa P(F_{i,j})\cdot\bfa P(F_{k,l})=O(\mu_n^2)$. Let $\gamma_n=O(\mu_n^2)$ and obtain the final result.
\end{proof}


==> sections/stochdeter.tex <==
In this subsection, we present the discussion over impossibility requirement of deterministic design. The method used here comes from the hypothesis testing problem on estimation within distribution family. Recall that for each vertices $i\in[n]$, the state space contains all possible outcome of comparisons with the rest $n-1$ parties. And we can see this problem as the estimation of the order of elements within a family of distribution induced by $M$. Asymptotically, if two elements are too close to each other, the estimation will fail due to the impossibility of distinguishing between them. Although a similar configuration is formed in ~\citet{shah2017simple}, our discussion does not focuses on lowerbounding the Minimax risk by the risk of an instance of testing problem. Instead, we are focusing on lowerbounding the risk of the test problem itself. The conditions of parameters for this problem can vary a lot. For example, ~\citet{shah2017simple} considers $\bar\Delta=\inf_{i\in[n-1]}\frac{1}{n}\sum_{k=1}^nM_{i,k}-\frac{1}{n}\sum_{k=1}^nM_{i+1,k}$ as an indicator of success for the top-k discovery.

Here state the following sufficient condition on the impossibility of exact ranking.
\begin{compactenum}
\item \textbf{Connectivity:} If the undirected random graph induced by $\ca A^m$ is unconnected with $\Omega(1)$ probability, the exact ranking will be impossible.
\item \textbf{Failure of the MAP Estimator:} If the MAP estimator failed with probability $\Omega(1)$, then the exact ranking will be impossible.
\end{compactenum}
\subsubsection{Connectivity}
In the seminal work by ~\citet{erdos1960evolution}. The connectivity of a single Erdős–Rényi graph $G(n,p)$ satisfies that when $p=\frac{\log n+c}{n}$
\begin{align*}
    \bfa P(G(n,p) \text{ is connected })\rightarrow e^{-e^{-c}}
\end{align*}
Then we analogously establishes the result for the ensembled random graphs $G^m(n,p)$ induced by $\ca A^m$
\begin{theorem}
When $p=\frac{\log n+c}{mn}$, $\bfa P(G^m(n,p)\text{ is connected })\rightarrow e^{-e^{-c}}$
\end{theorem}
\begin{proof}
The proof is straightforward once we observe that $G^m(n,p)$ is the same as $G(n,1-(1-p)^m)$
\end{proof}
And the above theorem directly implies the following:
\begin{corollary}
When $c>1$ and $p\geq \frac{c\log n}{mn}$, then the graph $G^m(n,p)$ is connected.
\end{corollary}
In the sequel, we only considered the situation where the graph is connected.
\subsubsection{Failure of MAP}
We start by analyzing the MAP estimator. Here we define the sample by $\bar{\bfa A}_1^m=\{\bbfa A^1,\ldots,\bbfa A^m\}$ We first decouple the generative procedure as follows: Assume that we have a Bernoulli random matrix $\bfa Q\in[0,1]^{n^2}$ defined by
\begin{align*}
    \bfa Q_{i,j}=\left\{\begin{matrix}
1 & \text{with probability } p \\
0 &  \text{with probability } 1-p\\
\end{matrix}\right.
\end{align*}
subjecting to $\bfa Q_{i,j} =\bfa Q_{j,i}$. Then we can decompose
$    \bbfa A=\bfa A\otimes \bfa Q$
where $\otimes$ is the element-wise product. Moreover, we see that for any $a>0$ :
\begin{equation*}
\bfa P(\bbfa A_{i,j}=a)=\bfa P(\bfa A_{i,j}=a,\bfa Q_{i,j}>0) =(1-p)\bfa P(\bfa A_{i,j}=a)
\end{equation*}
and $\bfa P(\bbfa A_{i,j}=0)=1-p$. We denote 
\begin{equation*}
    \ca A_{i,j}^{m,+}=\sum_{k=1}^m\bfa 1_{\bfa Q_{i,j}=1}\bfa 1_{\bfa A_{i,j}^k=1}\;\;\;\;\text{ and }\ca A_{i,j}^{m,-}=\sum_{k=1}^m\bfa 1_{\bfa Q_{i,j}=1}\bfa 1_{\bfa A_{i,j}^k=-1}
\end{equation*}
For simplicity of notation and without loss of generality, we can denote $\pi^*$ by the identity mapping.

As the result, we rewrite the maximum a posteriori criteria as
\begin{align*}
    \wh\pi_\text{MAP}&=\argmax_{\wh\pi\in\bb P}\bfa P(\Pi=\wh \pi|M,\bbfa A_1^m)\\
                     &=\argmax_{\wh\pi\in\bb P}\bfa P(\bbfa A_1^m|M, p,\Pi=\wh \pi)\bfa P(\Pi=\wh\pi)\\
                     &=\argmax_{\wh\pi\in\bb P}\prod_{k=1}^m\bfa P(\bbfa A^k|M,p,\Pi=\wh\pi)\bfa P(\Pi=\wh\pi)\\
                     &=\argmax_{\wh\pi\in\bb P}\sum_{k=1}^m\log(\bfa P(\bbfa A^k|M, p,\Pi=\wh \pi))\\
                     &=\argmax_{\wh\pi\in\bb P}\sum_{k=1}^m\sum_{i< j}^n\log(\bfa P(\bbfa A_{\wh \pi(i),\wh \pi(j)}|M_{ i, j},p,\Pi=\wh\pi))\\
                     &=\argmax_{\wh\pi\in\bb P}\sum_{k=1}^m\sum_{i<j:\bfa Q_{\pij}>0}\log(\bfa P(\bfa A_{\wh \pi(i),\wh \pi(j)}|M_{ i, j},p,\Pi=\wh\pi))
\end{align*}
According to the likelihood function of Binomial distribution, we see that when $i\neq j$
\begin{align*}
    \log(\bfa P(\bfa A_{i,j}|M_{i,j}))=\bfa A_{i,j}\cdot\log(M_{i,j})+(1-\bfa A_{i,j})\cdot\log(1-M_{i,j})
\end{align*}
% And we define $\log(\bfa P(\bfa A_{i,i}|M_{i,i}))=c$ for all $i\in[n]$.

Then we look into the objective that we maximize, recall that we denote the groundt truth to be $\pi^*$. For terms concerning $\wh\pi(i_1)$ and $\wh\pi(i_2)$, which is termed by $F(i_1,i_1) $ and $F(i_2,i_2)$, we define $F:\bb N\times\bb N\rightarrow\bb R^+$ as
\begin{align*}
    F(i,j)&=\sum_{k=1}^m\sum_{l\in [n]}\bfa 1_{\bfa Q_{\wh\pi(i),l}=1}\log(\bfa P(\bfa A_{\wh\pi(i),l}|M_{j,l},\Pi=\wh\pi))\\
    &=\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}\ca A_{\whp i,l}^{m,+}\log(M_{ j,l})+\ca A_{\whp i,l}^{m,-}\log(1-M_{ j,l})
\end{align*}
We can quickly identify a 'mixing error' $F(i_1,i_2)+F(i_2,i_1)\leq F(i_1,i_1)+F(i_2,i_2)$, given by
\begin{align*}
&\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}\bigg(\ca A_{\whp {i_1},l}^{m,+}\log(M_{ i_2,l})+\ca A_{\whp {i_2},l}^{m,+}\log(M_{ i_1,l})+\ca A_{\whp {i_1},l}^{m,-}\log(1-M_{ {i_2},l}) +\ca A_{\whp {i_2},l}^{m,-}\log(1-M_{ {i_1},l}) \bigg)\\
&\geq\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}\bigg(\ca A_{\whp {i_1},l}^{m,+}\log(M_{ i_1,l})+\ca A_{\whp {i_2},l}^{m,-}\log(M_{ i_2,l})+\ca A_{\whp {i_1},l}^{m,-}\log(1-M_{ {i_1},l}) +\ca A_{\whp {i_2},l}^{m,-}\log(1-M_{ {i_2},l})\bigg)
\end{align*}
which implies that
\begin{align*}
    E_{i_1,i_2}:=\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}(\ca A_{\whp {i_1},l}^{m,+}-\ca A_{\whp {i_2},l}^{m,+})\log\bigg(\frac{M_{{i_2},l}}{M_{{i_1},l}}\bigg)+(\ca A_{\whp {i_1},l}^{m,-}-\ca A_{\whp {i_2},l}^{m,-})\log\bigg(\frac{1-M_{{i_2},l}}{1-M_{{i_1},l}}\bigg)\geq 0
\end{align*}
We construct a random matrix $\bfa C^{(i_1,i_2)}\in\bb R^{2\times n}$ satisfies
\begin{align*}
 \text{ when $l\notin\{i_1,i_2\}$, }    \bfa C^{(i_1,i_2)}_{i_1,l}=\left\{\begin{matrix}
\log\big(\frac{M_{{i_2},l}}{M_{{i_1},l}}\big)& \text{with probability } M_{{i_1},l}p \\
\log\big(\frac{1-M_{{i_2},l}}{1-M_{{i_1},l}}\big) &  \text{with probability } (1-M_{{i_1},l})p\\
0& \text{ with probability } 1-p
\end{matrix}\right.
\end{align*}
and
\begin{align*}
 \text{ when $l\notin\{i_1,i_2\}$, }    \bfa C^{(i_1,i_2)}_{i_2,l}=\left\{\begin{matrix}
\log\big(\frac{M_{{i_1},l}}{M_{{i_2},l}}\big)& \text{with probability } M_{{i_2},l}p \\
\log\big(\frac{1-M_{{i_1},l}}{1-M_{{i_2},l}}\big) &  \text{with probability } (1-M_{{i_2},l})p\\
0& \text{ with probability } 1-p
\end{matrix}\right.
\end{align*}
In particular, we sample $m$ independent copies of $\bfa C^{(i_1.i_2)}$, denote by $\{\bfa C^{(1)},\ldots,\bfa C^{(m)}\}$, which is given by
\begin{equation*}
    \bfa P(E_{i_1,i_2}\geq 0)=\bfa P\big (\sum_{s\in[m]}\sum_{i\in\{i_1,i_2\}}\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}\bfa C^{(s)}_{i,l}\geq 0\big )
\end{equation*}
% Assuming $\whp {i_1}<\whp {i_2}$, we have the following sufficient condition:
% \begin{align*}
% \bfa P(E_1\geq 0)&\leq
%     \bfa P\bigg(\sum_{l\in [n]}(\ca A_{\whp {i_1},l}^{m,+}-\ca A_{\whp {i_2},l}^{m,+})\log\bigg(\frac{M_{{i_2},l}}{M_{{i_1},l}}\bigg)\geq 0\bigg)\\
%     &+\bfa P\bigg(\sum_{l\in [n]}(\ca A_{\whp {i_1},l}^{m,-}-\ca A_{\whp {i_2},l}^{m,-})\log\bigg(\frac{1-M_{{i_2},l}}{1-M_{{i_1},l}}\bigg)\geq 0
% \end{align*}
% or
% \begin{align*}
%     &E_1=\sum_{l\in [n]}(\ca A_{\whp {i_1},l}^{m,+}-\ca A_{\whp {i_2},l}^{m,+})\log\bigg(\frac{M_{{i_2},l}}{M_{{i_1},l}}\bigg)\geq 0\\
%     \text{ and }&E_2=\sum_{l\in [n]}(\ca A_{\whp {i_1},l}^{m,-}-\ca A_{\whp {i_2},l}^{m,-})\log\bigg(\frac{1-M_{{i_2},l}}{1-M_{{i_1},l}}\bigg)\geq 0
% \end{align*}
% Intuitively, we decouple the total event space into two subspaces, e.g. Wins and Losses.
First we review the following technical lemmas:
\begin{lemma}[Paley-Zygmund]
For random variable $Z>0$, for $\theta\in(0,1)$ we have
\begin{align*}
    \bfa P(Z\geq\theta\bb E[Z])\geq(1-\theta)^2\frac{\bb E[Z]^2}{\bb E[Z^2]}
\end{align*}
And for general random variable, we have
\begin{align*}
    \bfa P(\exp(tZ)\geq\theta\bb E[\exp(tZ)])\geq(1-\theta)^2\frac{\bb E[\exp(tZ)]^2}{\bb E[\exp(2tZ)]}
\end{align*}
\end{lemma}


which directly implies
\begin{corollary}[Second Order Method]
$
\bfa P(Z\geq 0)\geq\frac{\bb E[Z]^2}{\bb E[Z^2]}
$
\end{corollary}
and further implies
% \begin{corollary}
% Let $B_n=E_{1}\cup \cdots\cup E_{m(n)}$. where $E_{1},...,E_{m(n)}$ is a collection of events for each $n$. Write $i\overset{n}{\sim} j $ if $i\neq j$ and $E_{i}$ and $E_{j}$ are not independent. Then, letting
% \begin{equation*}
%     \mu_n:=\sum_{i=1}^{m(n)}\bfa P(E_{i}),\;\;\;\;\gamma_n:=\sum_{i\overset{n}{\sim}j}\bfa P(E_{i}\cap E_{j})
% \end{equation*}
% \label{cor1.2}
% where the second sum is over ordered pairs, we have $\lim_{n\rightarrow\infty}\bfa P(B_n)>0$ whenever $\mu_n\rightarrow\infty$ and $\gamma_n\leq C\mu_n^2$ for some $C>0$. If moreover $\gamma_n=o(\mu_n^2)$ then $\lim_{n\rightarrow\infty}\bfa P(B_n)=1$.
% \end{corollary}
The following lemma gives a sufficient condition of impossibility:
\begin{lemma}
Assume that $M_{i,j}=\Theta(1)$ as $n\rightarrow\infty$ (e.g. non-vanishing) and $|\sup_i (M_{i,i+1}-M_{i-1,i})|=\Delta \rightarrow 0$ as $n\rightarrow\infty$. If $\bfa P(E_{i,i+1}>0)=\Omega(\frac{1}{n})$ for all $i\in[n-1]$, then the exact ranking will be impossible.
\end{lemma}
\begin{proof}
Denote event $D_{i_1,i_2}: E_{i_1,i_2}\geq 0$. Let $(i_1,i_2)\overset{n}{\sim} (i_3,i_4)$ denote that $\bb E[D_{i_1,i_2}]\bb E[D_{i_3,i_4}]\neq\bb E[D_{i_1,i_2}\cap D_{i_3,i_4}]$. We also define the following quantities:
\begin{align*}
    \mu_n:=\sum_{i_1\neq i_2}^{n}\bfa P( D_{i_1,i_2})\;\;\;\;\gamma_n:=\sum_{(i_1,i_2)\overset{n}{\sim}(i_3,i_4)}\bfa P(D_{i_1,i_2}\cap D_{i_3,i_4})
\end{align*}
We denote $X_n:=\sum_{i_1\neq i_2}^n\bfa 1_{D_{i_1,i_2}}$. Note that
\begin{align*}
    Var[X_n]=\sum_{i_1\neq i_2}^n Var[\bfa 1_{D_{i_1,i_2}}]+\sum_{} Cov[\bfa 1_{D_{i_1,i_2}},\bfa 1_{D_{i_3,i_4}}]
\end{align*}
where
\begin{align*}
    Var[\bfa 1_{D_{i_1.i_2}}]=\bb E[(\bfa 1_{D_{i_1,i_2}})^2]-(\bb E[\bfa 1_{D_{i_1,i_2}}])^2\leq\bfa P(D_{i_1,i_2})
\end{align*}
In particular, when $D_{i_1,i_2}$ and $D_{i_3,i_4}$ are independent
\begin{align*}
    Cov[\bfa 1_{D_{i_1,i_2}},\bfa 1_{D_{i_3,i_4}}]=0
\end{align*}
whereas, if $(i_1,i_2)\overset{n}{\sim}(i_3,i_4)$,
\begin{align*}
    Cov[\bfa 1_{D_{i_1,i_2}},\bfa 1_{D_{i_3,i_4}}]=\bb E[\bfa 1_{D_{i_1,i_2}}\bfa 1_{D_{i_3,i_4}}]-\bb E[\bfa 1_{D_{i_1,i_2}}]\bb E[\bfa 1_{D_{i_3,i_4}}]\leq\bfa P(D_{i_1,i_2}\cap D_{i_3,i_4})
\end{align*}
Let $\bfa\Gamma=\sum_{s\in[m]}\bfa C^{(s)}_{i_1,i_3}+\bfa C^{(s)}_{i_1,i_4}+\bfa C^{(s)}_{i_2,i_3}+\bfa C^{(s)}_{i_2,i_4}$ be the sum of cross indices entries and note that $D_{i_1,i_2}\cap D_{i_3,i_4}$ can be rewritten according to the multiplicity of sub-indices by:
\begin{align*}
    &\bfa P(D_{i_1,i_2}\cap D_{i_3,i_4})-\bfa P(D_{i_1,i_2})\bfa P(D_{i_3,i_4})=\int \bfa P\big(D_{i_1,i_2}\cap D_{i_3,i_4}|\bfa\Gamma=c\big)\cdot\bfa P\big(\bfa\Gamma=c\big)dc-\bfa P(D_{i_1,i_2})\bfa P(D_{i_3,i_4})\\
    &=\int \bfa P(E_{i_1,i_2}\geq -c|\bfa\Gamma=c)\bfa P(E_{i_3,i_4}\geq -c|\bfa\Gamma=c)\bfa P(\bfa\Gamma=c)dc\\
    &=\int\bfa P(E_{i_1,i_2}\geq-c|\bfa\Gamma=c)(\bfa P(E_{i_3,i_4}\geq -c|\bfa\Gamma=c)-\bfa P(E_{i_3,i_4}>0))\bfa P(\bfa\Gamma=c)dc
\end{align*}
Note that as $n\rightarrow \infty$, the characteristic function satisifes:
\begin{align*}
    \bb E[\exp(it\bfa C_{i_1,l}+it\bfa C_{i_2,l})]=(1+O(it\Delta))\rightarrow 1
\end{align*}
This implies that
\begin{align*}
    \bb E[\exp(it\bfa\Gamma)]\rightarrow 1
\end{align*}
which further implies that
\begin{align*}
    \bb E[\exp(itE_{i_1,i_2})]\rightarrow\bb E[\exp(itE_{i_1,i_2})|\bfa\Gamma =d]
\end{align*}
According to the Inversion formula, we know that characteristic function uniquely determines probability density, which implies that
\begin{align*}
    \bfa P(E_{i_1,i_2}\geq-c|\Gamma=c)\overset{}{\rightarrow} \bfa P(E_{i_1,i_2}>0)
\end{align*}
Henceforth, as $n\rightarrow\infty$
\begin{equation*}
    \bfa P(D_{i_1,i_2}\cap D_{i_3,i_4})\rightarrow\bfa P(D_{i_1,i_2})\bfa P(D_{i_3,i_4})
\end{equation*}
Then we know that
 for any $i_1,i_2,i_3\in[n]$
\begin{align*}
    \bfa P(D_{i_1,i_2}\cap D_{i_2,i_3})\leq \min\{\bfa P(D_{i_1,i_2}), \bfa P(D_{i_2,i_3}\})=O(n)\bfa P(D_{i_1,i_2})\cdot\bfa P(D_{i_2,i_3})
\end{align*}
and we concluded by
\begin{align*}
    \gamma_n=O(\mu_n^2)
\end{align*}
We further note that using the condition in the Lemma, we have
\begin{align*}
    \frac{Var[X_n]}{(\bb E[X_n])^2}\leq\frac{\mu_n+\gamma_n}{\mu_n^2}=\frac{1}{\mu_n}+\frac{\gamma_n}{\mu_n^2}= O(1)
\end{align*}
And we finally have
\begin{align*}
    \bfa P(X_n>0)>\frac{(\bb EX_n)^2}{\bb E[X_n^2]}=\frac{(\bb EX_n)^2}{(\bb EX_n)^2+Var[X_n]}=\frac{1}{1+Var[X_n]/(\bb EX_n)^2}=\Omega(1)
\end{align*}
which implies impossibility.
\end{proof}
\begin{theorem}[Impossibility]
Assume that $M_{i,j}=\Theta(1)$ as $n\rightarrow\infty$. Let $\Delta_{i,j,l}=M_{i,l}-M_{j,l}$, then the following implies impossibility of exact ranking:
\begin{align*}
    \inf_{i,j}\sum_{l\in[n]\setminus\{i,j\}}\Delta^2_{i,j,l}\leq\frac{4\log n}{K_0mp}
\end{align*}
or, under a stricter condition
\begin{align*}
  \bar\Delta\leq\frac{2}{n}\sqrt{\frac{\log n}{K_0mp}}
\end{align*}
\end{theorem}
\begin{proof}
The proof follows from Paley-Zygmund inequality.
Let $\theta=\frac{1}{\bb E[\exp(tZ)]}$, we see that:
\begin{align*}
    \bfa P(Z\geq 0)=\bfa P(\exp(Z)\geq 1)\geq \bigg (1-\frac{1}{\bb E[\exp(tZ)]}\bigg)^2\frac{\bb E[\exp(tZ)]^2}{\bb E[\exp(2tZ)]}
\end{align*}
% \begin{lemma}
% Suppose $Z_1,\ldots,Z_k$ are i.i.d. $\bb E Z_i=0$ for all $i\in[k]$. Let $\phi_{Z_i}$ be the m.g.f. of $Z_i$. Suppose there exists constants $c_1,C_1>0$, such that
% \begin{equation*}
%     \exp(c_1t^2)\leq\phi_{Z_i}(t)\leq\exp(C_1t^2),\;\;\forall t\geq 0,1\leq i\leq k
% \end{equation*}
% then there exists constants $c, C>0$, such that for any fixed values $u_1,\ldots u_k\geq 0$, $X=u_1Z_1+\cdots+u_kZ_k$ satisfies
% \begin{equation*}
%     \bfa P(X\geq x)\geq c\exp(-\frac{-Cx^2}{\Vert u\Vert_2^2})
% \end{equation*}
% \end{lemma}
For the simplicity of notation, we denote
\begin{align*}
    \pa A_l=\frac{\tml}{\oml},\;\;\;\;\;\pa B_l=\frac{1-\tml}{1-\oml}
\end{align*}
And we note that $\log \pa A_l\cdot\log \pa B_l<0$ for all $\oml,\tml\in(0,1)$. In what follows, we assume $\log \pa A_l>0$, $\log\pa B_l<0$ and let $\bfa X_l\sim Bernoulli(\oml)$, $\bfa Y_l\sim Bernoulli(\tml)$ 

First we give the moment generating function for random variable $\bfa C_{i_1,l}^{(i_1,i_2)}$ by
\begin{align*}
    \psi_{\bfa C^{(i_1,i_2)}_{i_1,l}}(t)&=\bigg(\frac{\tml}{\oml}\bigg)^tp\oml+1-p+\bigg(\frac{1-\tml}{1-\oml}\bigg)^tp(1-\oml)\\
    &=\pa A_l^tp \oml+1-p+\pa B_l^tp(1-\oml)\\
    &=1-p+pD_{f_t}(\bfa X_l\Vert\bfa Y_l)
\end{align*}
where for $\bfa X_l\sim P$, $\bfa Y_l\sim Q$, we have that $D_{f_t}(\bfa X_l\Vert\bfa Y_l)=D_f(P\Vert Q)=\int (\frac{dP}{dQ})^tQ(dx)$ is the $f$-divergence with $f_t(x)=x^t$.

Similarly, for the random variable $\bfa C_{i_2,l}$, we see that
\begin{align*}
    \psi_{\bfa C^{(i_1,i_2)}_{i_2,l}}(t)&=\bigg(\frac{\oml}{\tml}\bigg)^tp\tml+1-p+\bigg(\frac{1-\oml}{1-\tml}\bigg)^tp(1-\tml)\\
    &=\pa A_l^tp \tml+1-p+\pa B_l^tp(1-\tml)\\
    &=1-p+pD_{f_t}(\bfa Y_l\Vert\bfa X_l)
\end{align*}% Also we note that
% \begin{align*}
%     \bb E[\bfa C_{i_1,l}]&=\log\pa A_l\oml+\log\pa B_l(1-\oml)\\
%     p_{1,l}:=\bb E[\bfa C^2_{1,l}]&=(\log\pa A_l)^2\oml+(\log \pa B_l)^2(1-\oml)\\
%     \bb E[\bfa C^3_{1,l+}]&=(\log\pa A_l)^3\oml\leq 3p_{1,l}c_{i,j}\\
%     \bb E[\bfa C^4_{1,l+}]&=(\log \pa A_l)^4\oml+(\log \pa B_l)^4(1-\oml)\leq 12p_{1,l}c_{i,j}^2\\
%     \text{ where }& c_{1,l}\leq\frac{\pa A_l}{3}\\
%     \bb E[\bfa C_{i_1,l+}^q]&=(\log \pa A_l)^q\oml+(\log\pa B_l)^q(1-\oml)\leq\frac{q!}{2}p_{1,l}c_{1.l}^{q-2}
% \end{align*}
% And we have 
% \begin{align}\label{eq}
%   p^tD^t_{KL}(\bfa X_l\Vert\bfa Y_l)&=\bigg(p\oml\pa A_l+p(1-\oml)\pa B_l\bigg)^t\leq\phi_{\bfa C_{i_1,l}}(t)
% \end{align}
% that comes from convexity.

Assembling pieces, we see that
\begin{align*}
    \bb E [\exp( tE_{i_1,i_2} )]&=\bb E[\exp (\sum_{i\in\{1,2\}}\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}t\bfa C_{i,l})]=\prod_{i\in\{1,2\}}\prod_{l\in[n]\setminus\{{i_1},{i_2}\}} \bb E[\exp(t\bfa C_{i,l})]
\end{align*}
which also yields that
\begin{align*}
    \bfa P(E_{i_1,i_2}> 0)>\frac{(\bb E[\exp(tE_{i_1,i_2})]-1)^2}{\bb E[\exp(2tE_{i_1,i_2})]}>\frac{\big (\prod_{s\in[m]}\prod_{i\in\{1,2\}}\prod_{l\in[n]\setminus\{{i_1},{i_2}\}}\bb E[\exp(t\bfa C^{(s)}_{i,l})]-1\big )^2}{\prod_{s\in[m]}\prod_{i\in\{1,2\}}\prod_{l\in[n]\setminus\{{i_1},{i_2}\}}\bb E[\exp(2t\bfa C^{(s)}_{i,l})]}
\end{align*}
Note that impossibility condition can be implied by:
\begin{align*}
    \bfa P(E_{i_1,i_2}>0)=\Omega \bigg(\frac{1}{n}\bigg)
\end{align*}
for all $i_2-i_1=1$. This is implied by
\begin{align*}
    \big(\prod_{s\in[m]}\prod_{i\in\{1,2\}}\prod_{l\in[n]\setminus\{{i_1},{i_2}\}}\bb E[\exp(t\bfa C_{i,l})]-1\big)^2=\Omega\bigg(\frac{1}{n}\prod_{s\in[m]}\prod_{i\in\{1,2\}}\prod_{l\in[n]\setminus\{{i_1},{i_2}\}}\bb E[\exp(2t\bfa C_{i,l})]\bigg)
\end{align*}
taking the logarithm over both side, we have
\begin{equation*}
    \sum_{s\in[m]}\sum_{i\in\{1,2\}}\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}(2\log(\bb E[\exp(t\bfa C_{i,l}^{(s)})]-1)-\log\bb E[\exp(2t\bfa C^{(s)}_{i,l})])\geq -\log n
\end{equation*}
Note that $\bb E[\exp(t\bfa C_{i_1,i_2})]\rightarrow 1$ as $n\rightarrow\infty$, the above can be implied by
\begin{align*}
    \frac{1}{n}\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}2\log(\bb E[\exp(t\bfa C_{i_1,l}+t\bfa C_{i_2,l})-1)-\log\bb E[\exp(2t\bfa C_{i_1,l}+2t\bfa C_{i_2,l})]\leq\frac{\log n}{nm}
\end{align*}
% Taking things together, and let $t\geq 1$ we found that above inequality can be implied by
% \begin{align*}
%     \frac{1}{n}\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}\log(1-p+pD_{f_t}(\bfa X_l\Vert\bfa Y_l))\leq\frac{\log n}{nm}
% \end{align*}
% or, taking the fact that $D_{f_t}(\bfa X_l\Vert\bfa Y_l)=1+o(1)$, we see that
% \begin{align*}
%   \frac{1}{n}\sum_{l\in[n]\setminus\{{i_1},{i_2}\}} p(D_{f_t}(\bfa X_l\Vert\bfa Y_l)-1)\leq\frac{\log n}{nm}
% \end{align*}
By the definition of $f_t$-divergence, let $\Delta_{i_1,i_2,l}=\oml-\tml$, we have
\begin{align*}
    D_{f_t}(\bfa X_l\Vert\bfa Y_l)&= \bigg(\frac{\tml}{\oml}\bigg)^t\oml+\bigg(\frac{1-\tml}{1-\oml}\bigg)^t(1-\oml)\\
    &=(\oml)^{-(t-1)}(\oml+\Delta_{i_1,i_2,l})^t+(1-\oml)^{-(t-1)}(1-\oml-\Delta_{i_1,i_2,l})^t\\
    &= (\oml)^{-(t-1)}(\oml^t+t\Delta_{i_1,i_2,l}\oml^{t-1}+\frac{1}{2}t(t-1)\Delta_{i_1,i_2,l}^2\oml^{t-2})\\
    &+(1-\oml)^{-(t-1)}[(1-\oml)^t-t\Delta_{i_1,i_2,l}(1-\oml)^{t-1}\\
    &+\frac{1}{2}t(t-1)\Delta_{i_1,i_2,l}^2(1-\oml)^{t-2})+o(\Delta_{i_1,i_2,l}^2)\\
    &=1+\frac{1}{2}t(t-1)(\oml^{-1}+(1-\oml)^{-1})\Delta_{i_1,i_2,l}^2+ o(\Delta_{i_1,i_2,l}^2)
\end{align*}
Collecting pieces, we concluded impossibility can be implied by
\begin{equation*}
    \frac{1}{n}\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}(-2t(2t-1))(\frac{1}{\oml}+\frac{1}{1-\oml})\Delta^2_{i_1,i_2,l}\leq \frac{\log n}{nm p}
\end{equation*}
Let $t=\frac{1}{4}$ and note that
\begin{align*}
    K_0:=\frac{1}{\gamma_{\max}}+\frac{1}{\gamma_{\min}}
\end{align*}
we finally conclude by
\begin{align*}
    \frac{K_0}{4}\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}\Delta_{i_1,i_2,l}^2\leq\frac{\log n}{mp}
\end{align*}
which completes the proof.
\end{proof}

\subsection{Information Theoretic Upperbound}
To obtain the information theoretic upperbound, we have the following lemma:
\begin{lemma}[Information Theoretic Achievability]
 If MAP estimator does not recover the ground truth, then with $\Theta (1)$ probability there exists $i_1,i_2\in[n]$ such that 
 \begin{align*}
     F(i_1,i_2)+F(i_2,i_1)\leq F(i_1,i_1)+F(i_2,i_2)
 \end{align*}
\end{lemma}

With this observation, we can see that:
\begin{theorem}
Assume that the probability is non-vaninshing, Let $\Delta_{i,j,l}=M_{i,l}-M_{j,l}$, then the following implies exact ranking of MLE estimator:
\begin{align*}
    \inf_{i,j}\sum_{l\in[n]}\Delta_{i,j,l}^2\geq\frac{K_0\log n}{4mp}
\end{align*}
Or under stricter condition:
\begin{align*}
    \bar\Delta\geq\sqrt{\frac{K_0\log n}{4nmp}}
\end{align*}
\end{theorem}
\begin{proof}
Let $\bfa X_{i,l}\sim Bernoulli(\bfa M_{i,l})$. We recall that the centered moment generating function of $\bfa C_{i_1,l}^{(i_1,i_2)}+\bfa C_{i_2,l}^{(i_1,i_2)}$ is
\begin{align*}
    \psi_{\bfa C_{i_1,l}^{(i_1,i_2)}+\bfa C_{i_2,l}^{(i_1,i_2)}}(t)&=\bb E[\exp(\bfa C_{i_1,l}^{(i_1,i_2)}+\bfa C_{i_2,l}^{(i_1,i_2)}-\bb E[\bfa C_{i_1,l}^{(i_1,i_2)}+\bfa C_{i_2,l}^{(i_1,i_2)}])]\\
    &=\bigg(\frac{M_{i_2,l}(1-M_{i_1,l})}{M_{i_1,l}(1-M_{i_2,l})}\bigg)^{tp(M_{i_2,l}-M_{i_1,l})}(1-p+pD_{f_t}(\bfa X_{i_1,l}\Vert\bfa X_{i_2,l})\\
    &\cdot(1-p+pD_{f_t}(\bfa X_{i_2,l}\Vert\bfa X_{i_1,l}))
\end{align*}
taking the logarithm over both side, we have
\begin{align*}
    \log\big(\psi_{\bfa C_{i_1,l}^{(i_1,i_2)}+\bfa C_{i_2,l}^{(i_1,i_2)}}(t)\big)&\leq\frac{t^2\delt^2p}{2}\bigg (\frac{1}{M_{i_1,l}}+\frac{1}{1-M_{i_1,l}}+\frac{1}{M_{i_2,l}}+\frac{1}{1-M_{i_2,l}}\bigg )+o(\delt^2)\\
    &\leq p\delt^2t^2\bigg(\frac{1}{\gamma_{\max}}+\frac{1}{\gamma_{\min}}\bigg)+o(\delt^2)
\end{align*}
By Bennet's inequality, we see that for $x\geq 0$
\begin{align*}
    \bfa P\bigg (\sum_{s\in[m]}\sum_{l\in[n]\setminus\{i_1,i_2\}}\bfa C_{i_1,l}^{(s)}+\bfa C_{i_2,l}^{(s)}-\bb E[\bfa C_{i_1,l}^{(s)}+\bfa C_{i_2,l}^{(s)}]\geq x\bigg )\leq\frac{\prod_{l\in[n]\setminus\{i_1,i_2\}}\psi_{\bfa C_{i_1,l}^{(i_1,i_2)}+\bfa C_{i_2,l}^{(i_1,i_2)}}(t)}{\exp (tx)}
\end{align*}
Let $K_0=\frac{1}{\gamma_{\max}}+\frac{1}{\gamma_{\min}}$.
By minimizing the R.H.S. we see that
\begin{align*}
   \bfa P\bigg (\sum_{s\in[m]}\sum_{l\in[n]\setminus\{i_1,i_2\}}\bfa C_{i_1,l}^{(s)}+\bfa C_{i_2,l}^{(s)}-\bb E[\bfa C_{i_1,l}^{(s)}+\bfa C_{i_2,l}^{(s)}]\geq x\bigg )\leq\exp\bigg(-\frac{x^2}{2pm\sum_{l\in[n]\setminus\{i_1,i_2\}} \delt^2K_0}\bigg)
\end{align*}
which gives us
\begin{align*}
    \bfa P(E_{i_1,i_2}\geq 0)&=\bfa P\bigg (\sum_{s\in[m]}\sum_{l\in[n]\setminus\{i_1,i_2\}}\bfa C_{i_1,l}^{(s)}+\bfa C_{i_2,l}^{(s)}-\bb E[\bfa C_{i_1,l}^{(s)}+\bfa C_{i_2,l}^{(s)}]\geq -m\sum_{l\in[n]\setminus\{i_1,i_2\}}\bb E[\bfa C_{i_1,l}^{(i_1,i_2)}+\bfa C_{i_2,l}^{(i_1,i_2)}]\bigg )\\
    &\leq\exp\bigg(-\frac{m^2(\sum_{l\in[n]\setminus\{i_1,i_2\}}\bb E[\bfa C_{i_1,l}^{(i_1,i_2)}+\bfa C_{i_2,l}^{(i_1,i_2)}])^2}{2pm\sum_{l\in[n]\setminus\{i_1,i_2\}} \delt^2K_0}\bigg)\\
    &\leq\exp\bigg(-\frac{8mp\sum_{l\in[n]\setminus\{i_1,i_2\}} \delt^2}{K_0}\bigg)
\end{align*}
where we applied the fact that when $\Delta_{i_1,i_2}\rightarrow 0$ and note that when $M_{i_1,l}$ and $M_{i_2,l}$ are on the same side of $\frac{1}{2}$
\begin{align*}
    \bb E[\bfa C_{i_1,l}^{(i_1,i_2)}+\bfa C_{i_2,l}^{(i_1,i_2)}]&=p(M_{i_2,l}-M_{i_1,l})\log\bigg(\frac{M_{i_2,l}(1-M_{i_1,l})}{M_{i_1,l}(1-M_{i_2,l})}\bigg)\\
    &\geq 4\delt^2p
\end{align*}
    We upperbound the joint event by the union bound:
    \begin{align*}
        \bfa P(\bigcup_{i_1,i_2\in[n]}E_{i_1,i_2})&\leq\sum_{i_1,i_2\in[n]:i_1\neq i_2}\bfa P(E_{i_1,i_2})\\
        &\leq\frac{n(n-1)}{2}\exp\bigg(-\frac{8mp\inf_{i,j}\sum_{l\in[n]\setminus\{i,j\}}\Delta_{i,j,l}^2}{K_0}\bigg)
    \end{align*}
    To guarantee consistency, we will only need:
    \begin{align*}
        \inf_{i,j}\sum_{l\in[n]\setminus\{i,j\}}\Delta^2_{i,j,l}\geq\frac{K_0\log n}{4mp}
    \end{align*}
    % And for a particular event $E_{i_1,i_2}$, recall that
    % \begin{align*}
    %     \bfa P(E_{i_1,i_2}\geq 0)
    %     &=\bfa P(\sum_{s\in[m]}\sum_{l\in[n]\setminus\{{i_1},{i_2}\}}\bfa C_{i_1,l}^{(s)}+\bfa C_{i_2,l}^{(s)}\geq 0)
    % \end{align*}
    %  Using the Chernoff bound and we have
    % \begin{align*}
    %     \bfa P(\sum_{s\in[m]}\sum_{l\in[n]\setminus\{i_1,i_2\}}\bfa  C_{i_1,l}^{(s)}+\bfa C_{i_2,l}^{(s)}\geq x)&\leq\exp(-xt)\cdot\prod_{l\in[n]\setminus\{i_1,i_2\}}\big (1-p+pD_{f_t}(\bfa X_{i_2,l}\Vert\bfa X_{i_1,l})\big)^m
    % \end{align*}
    % And we also note that
    % \begin{align*}
    %     1-p+pD_{f_t}(\bfa X_{i_2,l}\Vert\bfa X_{i_1,l})=1+\frac{1}{2}(t-1)t
    % \end{align*}
    % \begin{align*}
    %     \bfa P\bigg (\sum_{s\in[m]}\sum_{l\in[n]\setminus\{i_1,i_2\}}\bfa C_{i_1,l}^{(s)}+\bfa C_{i_2,l}^{(s)}\geq 0\bigg )&\leq\bb E[\exp(t\sum_{l\in[n]\setminus\{i_1,i_2\}}(\bfa C_{i_1,l}+\bfa C_{i_2,l})]\\
    %     &=\bigg(\prod_{l\in[n]\setminus\{{i_1},{i_2}\}}\big (1-p+pD_{f_t}(\bfa X_{i_2,l}\Vert\bfa X_{i_1,l})\big)\\
    %     &\cdot\big(1-p+pD_{f_t}(\bfa X_{i_1,l}\Vert\bfa X_{i_2,l})\big )\bigg)^{m-2}\\
    %     &\leq\prod_{l\in[n]\setminus\{i_1,i_2\}}\bigg (1-\frac{1}{2}\bigg)
    % \end{align*}
\end{proof}
% Hence, we see that:
% \begin{align*}
%     \bfa P\big (E_0\geq 0\big )&\geq\frac{(\bb E[\exp(tE_1)]-1)^2}{\bb E[\exp(2tE_1)]}\\
%                                  &=\frac{\big(\prod_{l\in[n]\setminus\{{i_1},{i_2}\}}\bb E[\exp t(\bbfa A_{\whp{i_1},l}-\bbfa A_{\whp{i_2},l})]-\prod_{l\in[n]\setminus\{{i_1},{i_2}\}}\big(\frac{M_{{i_2},l}}{M_{{i_1},l}}\big)^{-t}\big)^2}{\prod_{l\in[n]\setminus\{{i_1},{i_2}\}}\bb E\big[\exp(2t(\bbfa A_{\whp{i_1},l}-\bbfa A_{\whp{i_2},l}))\big]}
% \end{align*}
% The exact ranking in stochastic regime will induce more challenge. The introduction of parameter $p$ hence induce new challenges to the estimation of impossibility threshold. Instead of having a fixed number of comparisons for all vertices, the number of comparisons for each vertex follows a product of Binomial distributions. Here we studied the conditional Bayes estimation on a random matrix that can be represented by a matrix $\bfa T$ with $\bfa T_{i,j}+\bfa T_{j,i}\sim Binom(m, p)$ and $\bfa T_{i,j}$ is independent from other entries for all $i\neq j$. 
% \subsection{Impossibility}
% We note that by the probability distribution of $\bfa T$, the following lemma gives a necessary condition to exact ranking. This is a direct obervation from the fact that the parameter $p$ is not the sufficient statistics. (i.e. $\bfa P(\Pi|p)=\bfa P(\Pi)$)
% \begin{lemma}\label{impo2}
% Denote the ensembled comparison matrix by $\ca A^m$. We adopt the following normalization
% \begin{align*}
%     \oca_{i,j}=\frac{\ca A^m_{i,j}}{\ca A^m_{i,j}+\ca A^m_{i,j}}
% \end{align*}
% And the exact recovery is possible only when there exists non-trivial automorphism on $G$ that is induced by $\oca$ with probability $o(1)$
% \end{lemma}
% Lemma \ref{impo2} can be further weakened into the following general form:
% In a similar fashion, we 
% Denote $d_i$ by the number of comparisons concerning party $i$ in the $m$ rounds. Hence we are able to introduce $\bfa D=diag(d_1,...,d_n)$ as the diagonal degree matrix and a normalized comparison matrix defined as follows:
% \begin{equation*}
%     \bar{\ca A_{ij}^m}=\bfa D^{-\frac{1}{2}}\ca A_{ij}^m \bfa D^{-\frac{1}{2}}
% \end{equation*}
% We have the following claim regarding the MAP estimator in the stochastic setting:
% \begin{lemma}
% The MAP estimator will return identical estimation taking 
% \end{lemma}
% \begin{claim}
% Let $\ca A^{(i)}$ be the $i$-th column of the adjacency matrix $\ca A_{ij}^m$, then if there exists a constant $k\in\bb R^+$ such that $\ca A^{(i)}=k\cdot \ca A^{(j)}$, the exact ranking is not achievable by MAP, and hence not achievable by any algorithm.
% \end{claim}
% This claim can be further generalized similarly as in the deterministic setting.
% \begin{lemma}

% \end{lemma}
% % When multiple rounds of comparisons are generated according to $\bb M$, the learning context will be different in the sense that 
% % %, we are given a set of $m$ samples $\bfa A_1^m=\{\bfa A_1,...,\bfa A_m\}$ drawn from $\{0,1\}^{n\times n}$ i.i.d. Our objective is to recover the permutation $\pi$ such that the rank of $i$-th party is $\pi (i)$. Assume that we use some strategy with $\pi^*$ being its returned permutation when it takes $\bfa A_1^m$ as input and $\wh \pi$ be the ground truth. \lele{The relation between $\pi$ and $M$ is missing.}
% % The primary focus of this work is on the asymptotics of this problem, in other words, we want to study the fundamental question of \textbf{Under what conditions of parameters, will the ranking be successful with high probability as the scale of the problem goes to infinity ?} Formally, under what conditions on $\bfa M$, will the following holds
% % \begin{equation*}
% %     \bfa P_{\bfa M}(\wh\pi=\pi^*)\rightarrow 1 \text{ as } n\rightarrow \infty \text{ or } m\rightarrow\infty
% % \end{equation*}
% % in both the stochastic and full comparison setting.

% % \lele{Consider a collection of $n$ teams, indexed by $[n]:=\{1,\ldots,n\}$. 
% % % Let $\Pi^* : [n] \to [n]$ be a permutation over $[n]$. 
% % Let $M$ be an $n\times n$ a matrix satisfying the following properties.
% % \begin{itemize}
% %     \item For all $i,j \in [n]$, $0 \le M_{ij} \le 1$ and $M_{ij} + M_{ji}=1$;
% %     \item For all $i \neq j$, $\sum_{k = 1}^n M_{ik} \neq \sum_{k=1}^n M_{jk}$.
% % \end{itemize}
% % Here $M_{ij}$ indicates the probability that team $i$ wins over team $j$ in a match. Let $\Pi^*: [n] \to [n]$ the ranking of $sum_{k=1}^n M_{ik}$ for all $i \in [n]$. (TO BE DISCUSSED LATER.)

% % Suppose $m \in \mathbb{N^+}$ rounds of matches were played. In each round, between any pair of teams, with probability $p$, a match is played. In other words, for each pair $i>j$, let $N_{ij}$ be the number of matches played between teams $i$ and $j$. Then $N_{ij} \sim \mathrm{Binom}(m,p)$. Given $N_{ij}$, let $A_{ij} \sim \mathrm{Binom}(N_{ij}, M_{ij})$ and $A_{ji} = N_{ij} - A_{ij}$. We assume $A_{ii} = 0$ for all $i \in [n]$. In other words, among $N_{ij}$ matches played between teams $i$ and $j$, team $i$ wins $A_{ij}$ matches and team $j$ wins $A_{ji}$ matches.  In the special case when $p = 1$, $m$ matches are played between every pair of teams.

% % Suppose that the underlying permutation $\Pi^*$ and the probability matrix $M$ are unknown, only the match outcome matrix $A_n :=\{A_{ij}\}_{i,j \in [n]}$ is observed.  We wish to find an estimator $\hat{\Pi} = \hat{\pi}(A_n)$ that recovers the underlying permutation $\Pi^*$. 
% % % Assume $\Pi^*$ is uniform over all permutations over $[n]$. 
% % We say \emph{exact recovery is achievable} if there exists a sequence of estimators $\hat{\pi}(A_n)$ such that 
% % \[
% % \lim_{n \to \infty}\max_{\pi}\P(\hat{\Pi} \neq \Pi^*|\Pi^* = \pi) = 0.
% % \]
% % We say \emph{exact recovery is not possible} if for any estimator $\hat{\pi}(A_n)$, $\max_{\pi}\P(\hat{\Pi} \neq \Pi^*|\Pi^* = \pi) \nrightarrow 0$ as $n \to \infty$.}

% % \section{Methods}
% % Our method centered around the combinatorial threshold of random graphs induced by $\bfa A_1^m$. The induction goes by letting $\bb A$ be the adjacency matrix of the induced graph $\ca G_n$ with $\bb A_{ij}=\sum_{t=1}^m\bfa A_{ij}$. In particular, when $m=1$ we have $\bb A=\bfa A$. The following statement revealed a sufficient condition on successful recovery in single graph full comparision setting.
% % \begin{fact}
% % When there exists a pair $(i,j)$ such that the subgraph $\ca G_i,\ca G_j$ induced by $[n]\setminus i$ and $[n]\setminus j$ are isomorphic, then there are no algorithms that can recover the rank a.s. as $n\rightarrow\infty$. in the single round setting.
% % \end{fact}
% % which can be generalized to
% % \begin{fact} When there exists an non-trivial automorphism on the attributed graph $\ca G_n$ induced by $\bfa A_1^m$, then there exists no algorithm that can recover the rank a.s. as $n\rightarrow\infty$ or $m\rightarrow\infty$ in the multi round setting. 
% % \end{fact}

% % % \lele{Prove the two facts. Add the definition of automorphism on directed weighted graphs.}
% % To study the asymptotic with regard to $n$, we introduced a threshold function for this problem. Formally, a threshold function for a graph property $P$ is a function $r(n)$ such that:
% % \begin{equation*}
% %     \lim_{n\rightarrow\infty}\bfa P_{\bfa M}[\ca G_n \text{ has property P}]=\left\{\begin{matrix}
% %  0&\;\;\text{ if }p_n\ll r(n) \\ 
% %  1& \;\;\text{ if } p_n\gg r(n)
% % \end{matrix}\right.
% % \end{equation*}
% % The following inequalities served as the preliminaries of our method.

% % \section{Results}
% % We first present the result of full comparison in a single round, then move on to the more complicated stochastic comparisons of single/multiple rounds.
% % The following lemma stated the result of single round full comparison .
% % \begin{theorem}
% % Under the \textit{Single Round Full Comparision} setting, no algorithm will be able to recover the rank when there exists $i,j$ such that $M_{i,j}=\frac{1}{2}$
% % \end{theorem}
% % \begin{proof}
% % Using corollary \ref{cor1.2}, we define 
% % \begin{equation*}
% %     A_{i,j}=\{  \bb A_{i,k}=\bb A_{j,k} \text{ for all }k\in[n]\text{ with }i\neq j\text{ , }i\neq k\text{ and } j\neq k \}
% % \end{equation*} which is the event such that $i$ and $j$ is not distinguishable in the induced random graph.
% % And we immediately have
% % \begin{equation*}
% %     \bfa P(A_{i,j})=\frac{1}{4}\sum_{\bfa X\in\{0,1\}^{n}}\prod_{k\in[n]\setminus \{i,j\}}(M_{ik}M_{jk})^{\bfa X_k}(1-M_{ik})^{(1-\bfa X_k)}(1-M_{jk})^{(1-\bfa X_k)}
% % \end{equation*}
% % Hence,
% % \begin{equation*}
% %     \mu_n=\frac{1}{4}\sum_{i,j\in[n],i\neq j}\sum_{\bfa X\in\{0,1\}^{n}}\prod_{k\in[n]\setminus \{i,j\}}(M_{ik}M_{jk})^{\bfa X_k}(1-M_{ik})^{(1-\bfa X_k)}(1-M_{jk})^{(1-\bfa X_k)}
% % \end{equation*}
% % where the constant $\frac{1}{4}$ comes from the fact that $\bfa X_i$ and $\bfa X_j$ are redundant.
% % Since $ A_{ij}\bot A_{kl}$ when $\{i,j\}\cap\{k,l\}=\emptyset$, the correlation only exists when $card(\{i,j\}\cup\{l,k\})\leq 3$, without loss of generality, we have
% % \begin{align*}
% % \bfa P(A_{i,j}\cup A_{k,j})&=\bfa P(A_{i,j}\cup A_{j,k}) \\
% % &=\frac{1}{4}\sum_{\bfa X\in\{0,1\}^n}\prod_{m\in[n]\setminus\{i,j,k\}}(M_{i,m}M_{j,m}M_{k,m})^{\bfa X_m}\\
% % &\bigg((1-M_{i,m})(1-M_{j,m})(1-M_{j,m})\bigg)^{(1-\bfa X_m)}(M_{i,k}M_{i,j}M_{j,k})^{\bfa X_i}\\
% % &\bigg((1-M_{i,k})(1-M_{j,k})(1-M_{i,j})\bigg)^{(1-\bfa X_i)}\\
% % \end{align*}
% % Hence
% % \begin{align*}
% %     \gamma_n=\sum_{i,j,k\text{ non-identical to each other}}\bfa P(A_{i,j}\cup A_{k,j})
% % \end{align*}
% % Define the union $B=\bigcup_{i,j\in[n],i\neq j}A_{i,j}$, and a sufficient condition of $\bfa P(B)>0$ will be:
% % \begin{equation*}
% %     \gamma_n=O(\mu_n^2)
% % \end{equation*}
% % Then the threshold equality became:
% % \begin{equation*}
% %     \gamma_n=C\mu_n^2
% % \end{equation*}
% % % We use the Fourier-Walsh expansion on Boolean functions. By rewriting $\mu_n$ as:
% % % \begin{align*}
% % %     \mu_n&=\frac{1}{4}\sum_{i,j\in[n],i\neq j}\sum_{\bfa X\in\{-1,1\}^{n}}\prod_{k\in[n]\setminus \{i,j\}}(M_{ik}M_{jk})^{(1+\bfa X_k)/2}(1-M_{ik})^{(1-\bfa X_k)/2}(1-M_{jk})^{(1-\bfa X_k)/2}
% % %     % &=2^{n-2}\bb E[\sum_{S\subset\{1,...,n\}}\alpha_Su_S(\bfa X)]
% % % \end{align*}
% % % with 
% % % \begin{equation*}
% % %     u_S(\bfa X)=\prod_{i\in S}\bfa X_i
% % % \end{equation*}
% % % and define the inner product by
% % % \begin{equation*}
% % %     \langle f,g\rangle=2^{-n}\sum_{\bfa X\in\{-1,1\}^n}f(\bfa X)g(\bfa X)
% % % \end{equation*}
% % % then it is immediate to see that for any $S,S^\prime\subset\{1,...,n\}$,
% % % \begin{equation*}
% % %     \langle u_S,u_{S^\prime}\rangle=\left\{\begin{matrix}
% % % 0 &\text{ if } S\neq S^\prime \\ 
% % % 1 &\text{ if } S=S^\prime 
% % % \end{matrix}\right.
% % % \end{equation*}
% % % Hence we can generate the coefficients by
% % % \begin{equation*}
% % %     \alpha_S=\langle
% % % \end{equation*}
% % \begin{align*}
% %     \mu_n^2&=\frac{1}{16}\bigg(\sum_{\bfa X\in\{0,1\}^n}\prod_{k\in[n]\setminus\{ i,j\}}(M_{ik}M_{jk})^{\bfa X_k}(1-M_{ik})^{(1-\bfa X_k)}(1-M_{jk})^{(1-\bfa X_k)}\bigg)^2\\
% %     &=\frac{1}{16}\sum_{\bfa X\in\{0,1\}^n}\prod_{k\in[n]\setminus\{ i,j\}}(M_{ik}M_{jk})^{\bfa X_k}(1-M_{ik})^{(1-\bfa X_k)}(1-M_{jk})^{(1-\bfa X_k)}
% % \end{align*}
% % \end{proof}






